Concurrent Composition of Differential Privacy

We initiate a study of the composition properties of interactive differentially private mechanisms. An interactive differentially private mechanism is an algorithm that allows an analyst to adaptively ask queries about a sensitive dataset, with the property that an adversarial analyst's view of the interaction is approximately the same regardless of whether or not any individual's data is in the dataset. Previous studies of composition of differential privacy have focused on non-interactive algorithms, but interactive mechanisms are needed to capture many of the intended applications of differential privacy and a number of the important differentially private primitives. We focus on concurrent composition, where an adversary can arbitrarily interleave its queries to several differentially private mechanisms, which may be feasible when differentially private query systems are deployed in practice. We prove that when the interactive mechanisms being composed are pure differentially private, their concurrent composition achieves privacy parameters (with respect to pure or approximate differential privacy) that match the (optimal) composition theorem for noninteractive differential privacy. We also prove a composition theorem for interactive mechanisms that satisfy approximate differential privacy. That bound is weaker than even the basic (suboptimal) composition theorem for noninteractive differential privacy, and we leave closing the gap as a direction for future research, along with understanding concurrent composition for other variants of differential privacy.

==> approxDP.tex <==
In this section, we explore the privacy guarantee for the concurrent composition of interactive differential privacy when $\delta > 0$.
%\section{Group Privacy-Like Bound}
We show a privacy guarantee of concurrent composition in a similar logic flow as in Theorem \ref{thm:concomp-basic}, but in approximate differential privacy. 
As argued in the proof of Theorem \ref{thm:concomp-basic}, when the adversary is interacting with two mechanisms, we can view $\analyst$ and one of the mechanisms as a single adversary interacting with another mechanism, and the view of the combined adversary still enjoy the differential privacy guarantee. Therefore, if both interactive mechanisms $\mechanism$ and $\Tilde{\mechanism}$ are $(\eps, \delta)$-differentially private, then for all $S \subseteq \range(\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))})$, 
we know that 
\begin{align}
& \Pr \left[
\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \in S \right] \nonumber \\
& \le e^\eps \Pr \left[
\view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \in S \right] + \delta \nonumber
\end{align}
and 
\begin{align}
& \Pr \left[
\view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \in S \right] \nonumber \\
& \le e^\eps \Pr \left[
\view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x'))} \in S \right] + \delta  \nonumber
\end{align}
and therefore we know that 
\begin{align}
& \Pr \left[
\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \in S \right] \nonumber \\
& \le e^\eps \Pr \left[
\view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \in S \right] + \delta \nonumber \\
& \le e^\eps (e^\eps \Pr \left[
\view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x'))} \in S \right] + \delta ) + \delta \nonumber \\
& \le e^{2\eps} \Pr \left[
\view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x'))} \in S \right] 
+ (1+e^\eps) \delta \nonumber
\end{align}

%\begin{theorem}
%If interactive mechanisms $\mechanism_0, \dots, \mechanism_{k-1}$ are each $(\eps_i, \delta_i)$-differentially private, then their concurrent composition $\concomp(\mechanism_0, \ldots, \mechanism_{k-1})$ is $(\sum_{i=0}^{k-1} \eps_i, k e^{\sum_{i=0}^{k-1} \eps_i} \max_i(\delta_i))$ differentially private. 
%\end{theorem}
A more general concurrent composition bound is stated and derived as follows:
\concompbasicapprox*
\begin{proof}
We use a hybrid argument. For each $0 \le i \le k-1$, since $\mechanism_i$ is $(\eps_i, \delta_i)$ differentially private, we know that 
\begin{align}
& \Pr \left[
\view{\analyst}{\concomp(\mechanism_0(x'), \ldots,  \mechanism_{i-1}(x'), \mechanism_{i}(x), \ldots, \mechanism_{k-1}(x))} \in S \right] \nonumber \\
& \le e^{\eps_i}
\Pr \left[
\view{\analyst}{\concomp(\mechanism_0(x'), \ldots,  \mechanism_{i-1}(x'), \mechanism_{i}(x'), \ldots, \mechanism_{k-1}(x))} \in S \right] + \delta_i \nonumber
\end{align}
by viewing $\analyst$ and $\mathcal{M}_0, \dots, \mathcal{M}_{i-1}, \mathcal{M}_{i+1},  \mathcal{M}_{k-1}$ as a combined adversary and follow a similar argument as in the proof of Theorem \ref{thm:concomp-basic-approx}. 

Therefore, 
\begin{align}
& \Pr \left[
\view{\analyst}{\concomp(\mechanism_0(x), \mechanism_1(x), \ldots, \mechanism_{k-1}(x))} \in S \right] \nonumber \\
& \le e^{\eps_0}
\Pr \left[
\view{\analyst}{\concomp(\mechanism_0(x'), \mechanism_1(x), \ldots, \mechanism_{k-1}(x))} \in S \right] + \delta_0 \nonumber \\
& \le e^{\eps_0}
(e^{\eps_1}
\Pr \left[
\view{\analyst}{\concomp(\mechanism_0(x'), \mechanism_1(x'), \ldots, \mechanism_{k-1}(x))} \in S \right] + \delta_1) + \delta_0 \nonumber \\
& \le \ldots \nonumber \\
& \le e^{\sum_{i=0}^{k-1} \eps_i} 
\Pr \left[
\view{\analyst}{\concomp(\mechanism_0(x'), \mechanism_1(x'), \ldots, \mechanism_{k-1}(x'))} \in S \right] \nonumber \\
&~~~~+ (\delta_0+e^{\eps_0}\delta_1  + e^{\eps_0+\eps_1} \delta_2 + \ldots + e^{\sum_{i=0}^{k-2} \eps_i}\delta_{k-1} ) \nonumber 
\end{align}
We can see that the $\delta$ term of $\concomp(\mechanism_0, \ldots, \mechanism_{k-1})$ depends on different permutations of $(\mechanism_0, \ldots, \mechanism_{k-1})$, and the tightest possible bound for the $\delta$ term is 
$$
\min_{\sigma} 
\left( 
\delta_{\sigma(0)} + \sum_{i=1}^{k-1} e^{\sum_{j=0}^{i-1}\eps_{\sigma(j)}} \delta_{\sigma(i)} 
\right)
$$
We also note that $\delta_0+e^{\eps_0}\delta_1  + e^{\eps_0+\eps_1} \delta_2 + \ldots + e^{\sum_{i=0}^{k-2} \eps_i}\delta_{k-1} \le k e^{\sum_{i=0}^{k-1} \eps_i} \max_i (\delta_i)$, which is more easier to work with in practice. 
\end{proof}

Notice that if the privacy parameters are homogeneous, i.e. every interactive mechanism is $(\eps, \delta)$ differentially private, then this bound reduce to the bound of group privacy for $(\eps, \delta)$-differential privacy. 



==> characterization.tex <==
%\section{Characterization of $\concomp$}

\cite{kairouz2015composition} shows that to analyze the composition of arbitrary non-interactive $(\eps_i, \delta_i)$-DP algorithms, it suffices to analyze the composition of the following simple variant of randomized response. 

\newcommand{\iamzero}{\texttt{`Iam0'}}
\newcommand{\iamone}{\texttt{`Iam1'}}

\begin{definition}[\cite{kairouz2015composition}]
Define a randomized non-interactive algorithm 
$\RR_{(\eps, \delta)}:\{0,1\} \rightarrow\{0,1, \iamzero , \iamone \}$ as follows:
$$
\begin{array}{ll}
\operatorname{Pr}\left[\RR_{(\eps, \delta)}(0)=\iamzero \right]=\delta & \operatorname{Pr}\left[\RR_{(\eps, \delta)}(1)=\iamzero \right]=0 \\
\operatorname{Pr}\left[\RR_{(\eps, \delta)}(0)=0\right]= (1-\delta) \cdot \frac{e^{\eps}}{1+e^{\eps}} & \operatorname{Pr}\left[\RR_{(\eps, \delta)}(1)=0\right]= (1-\delta) \cdot \frac{1}{1+e^{\eps}} \\
\operatorname{Pr}\left[\RR_{(\eps, \delta)}(0)=1\right]= (1-\delta) \cdot \frac{1}{1+e^{\eps}} & \operatorname{Pr}\left[\RR_{(\eps, \delta)}(1)=1\right]= (1-\delta) \cdot \frac{e^{\eps}}{1+e^{\eps}} \\
\operatorname{Pr}\left[\RR_{(\eps, \delta)}(0)=\iamone \right]=0 & \operatorname{Pr}\left[\RR_{(\eps, \delta)}(1)=\iamone \right]=\delta
\end{array}
$$
\end{definition}
Note that $\RR_{(\eps, \delta)}$ is a non-interactive $(\eps, \delta)$-differentially private mechanism. \cite{kairouz2015composition} and \cite{murtagh2016complexity} showed that $\RR_{(\eps, \delta)}$ can be used to simulate the output of every (non-interactive) $(\eps, \delta)$-DP algorithm on adjacent databases. $\RR$ refers to ``randomized response", as this mechanism mimics the classic randomized response \citep{warner1965randomized}. 

\begin{theorem}[\cite{kairouz2015composition}]
\label{thm:noninterac}
Suppose that $\mechanism$ is $(\eps, \delta)$-differentially private. Then for every pair of adjacent datasets $x_0, x_1$ there exists a randomized algorithm $T$ s.t. $T(\RR (b))$ is identically distributed to $\mechanism(x_b)$ for both $b=0$ and $b=1$. 
%, where RR is $(\eps, \delta)$-randomized response as below. 
\end{theorem}

%\todo{also give formulation in terms of events}

In non-interactive setting, Theorem \ref{thm:noninterac} can be used to prove the optimal composition theorem \citep{kairouz2015composition, murtagh2016complexity} since to analyze the composition of arbitrary $(\eps_i, \delta_i)$-DP algorithms, it suffices to analyze the composition of $\RR_{(\eps_i, \delta_i)}$ algorithms. 
If we are able to prove a similar result that arbitrary interactive differential private mechanisms can also be simulated by the post-processing of randomized response where the interactive post-processing algorithm does not depend on the adversary, then we will be able to extend all results of composition theorem for non-interactive mechanisms to interactive mechanisms. In this paper, we consider the case of pure differential privacy. 

%\todo{formalize interactive post-processing mechanism}

\begin{theorem}
\label{thm:reduction-pure}
Suppose that $\mechanism$ is an interactive $(\eps, 0)$-differentially private mechanism. Then for every pair of adjacent datasets $x_0, x_1$ there exists an interactive mechanism $T$ s.t. for every adversary $\analyst$ and every $b \in \{0, 1\}$ we have 
\begin{equation}
\View(\analyst, \mechanism(x_b))
    \equiv \View(\analyst, T(\RR_{(\eps, 0)}(b))) \nonumber
\end{equation}
\end{theorem}

\begin{proof}
For arbitrary sequence of queries $\bm{q}^{(t)} = (q_0, \dots, q_{t-1})$ from $\analyst$, 
we denote by
$
\vec{\mechanism}(x, \bm{q}^{(t)}) = 
(\mechanism(x, \bm{q}^{(1)}), \mechanism(x, \bm{q}^{(2)}), \dots, \mechanism(x, \bm{q}^{(t)}))
$
the random variable consisting the first $t$ responses from mechanism $\mechanism$. 
We construct the interactive mechanism $T$ receiving queries $\bm{q}^{(t)}$ as follows: 
\begin{enumerate}
    \item If $t=0$, we have
    \begin{equation}
    \begin{split}
    \Pr \left[ T(0, q_0)=a_0 \right] = \frac{ e^\eps \Pr[\mechanism(x_0, q_0)=a_0] - \Pr[\mechanism(x_1, q_0)=a_0] }{e^\eps - 1}
    \end{split}
    \end{equation}
    \begin{equation}
    \begin{split}
    \Pr \left[ T(1, q_0)=a_0 \right] = \frac{ e^\eps \Pr[\mechanism(x_1, q_0)=a_0] - \Pr[\mechanism(x_0, q_0)=a_0] }{e^\eps - 1}
    \end{split}
    \end{equation}
    \item If $t>0$, given earlier responses $(a_0, \dots, a_{t-2})$, we define 
    \begin{equation}
    \begin{split}
    &\Pr \left[ T(0, \bm{q}^{(t)}) = a_{t-1} | a_0, \dots, a_{t-2} \right] \\
    &= \frac{e^\eps \Pr \left[ \vec{\mechanism}(x_0, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) \right] - \Pr \left[ \vec{\mechanism}(x_1, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) \right] }{(e^\eps - 1) \Pr \left[ \vec{T}(0, \bm{q}^{(t-1)}) = (a_0, \dots, a_{t-2}) \right] }
    \label{eq:dist-post}
    \end{split}
    \end{equation}
    \begin{equation}
    \begin{split}
    &\Pr \left[ T(1, \bm{q}^{(t)}) = a_{t-1} | a_0, \dots, a_{t-2} \right] \\
    &= \frac{e^\eps \Pr \left[\vec{\mechanism}(x_1, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) \right] - \Pr \left[\vec{\mechanism}(x_0, \bm{q}^{(t)})=(a_0, \dots, a_{t-1})\right] }{(e^\eps - 1) \Pr \left[\vec{T}(1, \bm{q}^{(t-1)}) = (a_0, \dots, a_{t-2})\right] }
    \end{split}
    \end{equation}
\end{enumerate}

Therefore, the distribution of $\vec{T}$ is 
\begin{align}
    &\Pr \left[ \vec{T}(0, \bm{q}^{(t)}) = (a_0, \dots, a_{t-1}) \right] \nonumber \\
    &= \frac{e^\eps \Pr \left[\vec{\mechanism}(x_0, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) \right] - \Pr \left[\vec{\mechanism}(x_1, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) \right] }{e^\eps - 1} \nonumber
\end{align}
\begin{align}
    &\Pr \left[ \vec{T}(1, \bm{q}^{(t)}) = (a_0, \dots, a_{t-1}) \right] \nonumber \\
    &= \frac{e^\eps \Pr \left[\vec{\mechanism}(x_1, \bm{q}^{(t)})=(a_0, \dots, a_{t-1})\right] - \Pr \left[\vec{\mechanism}(x_0, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) \right] }{e^\eps - 1} \nonumber
\end{align}

We can easily verify that all of the above are valid probability distributions. 
For example, 
\begin{align}
    &\sum_{a_{t-1}} \Pr \left[ T(0, \bm{q}^{(t)}) = a_{t-1} | a_0, \dots, a_{t-2} \right] \nonumber \\
    &= \frac{e^\eps \sum_{a_{t-1}} \Pr \left[ \vec{\mechanism}(x_0, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) \right] - \sum_{a_{t-1}} \Pr \left[ \vec{\mechanism}(x_1, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) \right] }{(e^\eps - 1) \Pr \left[ \vec{T}(0, \bm{q}^{(t-1)}) = (a_0, \dots, a_{t-2}) \right] } \nonumber \\
    & = \frac{e^\eps \Pr \left[ \vec{\mechanism}(x_0, \bm{q}^{(t)})=(a_0, \dots, a_{t-2}) \right] -  \Pr \left[ \vec{\mechanism}(x_1, \bm{q}^{(t)})=(a_0, \dots, a_{t-2}) \right] }{(e^\eps - 1) \Pr \left[ \vec{T}(0, \bm{q}^{(t-1)}) = (a_0, \dots, a_{t-2}) \right] } \nonumber \\
    & = 1
\end{align}
and for every possible $a_{t-1}$, the probability density is never negative since 
$$
\Pr \left[ \vec{\mechanism}(x_0, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) \right]
\le e^\eps \Pr \left[ \vec{\mechanism}(x_1, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) \right]
$$
as $\mechanism$ is $(\eps, 0)$-DP. 

%Given any transcript $(a_0, \dots, a_{t-1})$ and the randomness $r$ of $\analyst$, we can derive the queries asked by $\analyst$ by computing 
%$$
%q_i = \analyst(a_0, \dots, a_{i-1}; r)
%$$
%for all $i \le t-1$. 

We now show 
$$
\View(\analyst, \mechanism(x_b))
    \equiv \View(\analyst, T(\RR_{(\eps, 0)}(b)))
$$
for the case of $b=0$. 

Fix any possible view $(r, a_0, \dots, a_{t-1})$, we can derive the queries $\bm{q}^{(t)} = (q_0, \ldots, q_{t-1})$ from $\analyst$, where $q_i = \analyst(a_0, \ldots, a_{i-1}; r)$. 
\begin{align}
&\Pr \left[ \View(\analyst, T(\RR_{(\eps, 0)}(0))) = (r, a_0, \dots, a_{t-1}) \right] \nonumber \\
& = \Pr \left[\RR_{(\eps, 0)}(0)=0 \right] \Pr \left[ \View(\analyst, T(0)) = (r, a_0, \dots, a_{t-1}) \right] \nonumber \\
&~~~~+ \Pr \left[\RR_{(\eps, 0)}(1)=0 \right] \Pr \left[ \View(\analyst, T(1)) = (r, a_0, \dots, a_{t-1}) \right] \nonumber \\
& = \frac{e^\eps}{1+e^\eps} \Pr \left[ \View(\analyst, T(0)) = (r, a_0, \dots, a_{t-1}) \right] \nonumber \\
&~~~~+ \frac{1}{1+e^\eps} \Pr \left[ \View(\analyst, T(1)) = (r, a_0, \dots, a_{t-1}) \right] \nonumber \\
& = \frac{e^\eps}{1+e^\eps} \left[ R=r \right]
\Pr \left[ \vec{T}(0, \bm{q}^{(t)}_r) = (a_0, \dots, a_{t-1})  | R=r \right] \nonumber \\
&~~~~+ \frac{1}{1+e^\eps} \left[ R=r \right] 
\Pr \left[ \vec{T}(1, \bm{q}^{(t)}_r) = (a_0, \dots, a_{t-1}) | R=r \right] \nonumber \\
& = \Pr \left[ R=r \right] \Pr \left[\vec{\mechanism}(x_0, \bm{q}^{(t)}_r)=(a_0, \dots, a_{t-1}) | R=r \right]
 \nonumber \\
& = \Pr \left[\View(\analyst, \mechanism(x_0)) = (a_0, \dots, a_{t-1}) \right] \nonumber
\end{align}
The case of $b=1$ could be similarly proved. Therefore, we proved the existence of such an interactive mechanism $T$ for any $(\eps, 0)$ interactive DP mechanisms. 
\end{proof}


\begin{comment}
\section{Interactive Mechanism}
An interactive mechanism $\mechanism$ is a randomized function that takes a private dataset $x \in \mathcal{X}^n$, and then spawns a (possibly randomized) state machine $Q=\mechanism(x)$ called \emph{queryable}. The queryable consists of an initial private state $s_0$, and an evaluation function Eval. It then receives a query $q_1$. Based on $q_1$ and current state $s_0$, it generates a possibly randomized response $a_1$ and updates its private state to $s_1$. That is, $(a_1, s_1) \leftarrow Eval(q_1, s_0)$. It then receives $q_2$, and generate response and new state, so and so forth. The interactive session can be arbitrarily long. 

We consider an arbitrary adversarial strategy $\analyst$ interacting with $\mechanism(x)$, which selects each query $q_i$ based on all previous responses $(a_1, \dots, a_{i-1})$ and the randomness of $\analyst$. 
Let $View(\analyst \leftrightarrow \mechanism(x))$ be a random variable denoting $\analyst$'s view of this entire interaction. 
$$
View(\analyst \leftrightarrow \mechanism(x)) = (R, A_1, A_2, \dots,)
$$
\begin{definition}
For $\eps, \delta \ge 0$, we say $\mechanism$ is $(\eps, \delta)$-DP interactive mechanism if for every $x \sim x'$, for every strategy $\analyst$, let 
$Y=\view{\analyst}{\mechanism(x)}$ and $Y' = \view{\analyst}{\mechanism(x')}$, we have 
$$
\forall T\in \mathcal{Y},~
Pr[Y \in T] \le e^\eps Pr[Y' \in T] + \delta
$$
\end{definition}

Note that we can easily write the probability of getting a transcript $y=(r, a_1, a_2, \dots, )$ in conditional probability form:
$$
Pr[\view{\analyst}{\mechanism(x)}=(r, a_1, a_2, \dots, )]
= Pr[R=r]Pr[A_1=a_1|r]Pr[A_2=a_2|r, a_1] \dots
$$

For $(\eps, 0)$-DP interactive mechanism $\mechanism$, the definition is equivalent to: for every $x \sim x'$, for every strategy $\analyst$, for all transcript $y=(r, a_1, a_2, \dots)$, we have 
\begin{align}
    \log(\frac{Pr[\view{\analyst}{\mechanism(x)}=(r, a_1, a_2, \dots, )]}{Pr[\view{\analyst}{\mechanism(x')}=(r, a_1, a_2, \dots, )]})
    &=
    \log(\frac{Pr[R=r]Pr[A_1=a_1|r]Pr[A_2=a_2|r, a_1] \dots}{Pr[R=r]Pr[A_1'=a_1|r]Pr[A_2'=a_2|r, a_1] \dots}) \\
    &= \sum_{i=1}^{\infty}
    \log(\frac{Pr[A_i=a_i|r, a_1, \dots, ]}{Pr[A_i'=a_i|r, a_1, \dots, ]})
    \le \eps
\end{align}
i.e. the sum of privacy loss for each message is less than or equal to $\eps$. 

\end{comment}

%\subsection{Connection with Non-interactive mechanism: approximate DP case

\begin{comment}


We then discuss the case when $\delta > 0$. 
%In \cite{murtagh2016complexity}, it shows that every (non-interactive) $(\eps, \delta)$-DP mechanism is the post-processing of a randomized response. The key idea of proving this claim is by conditioning on some special events and making reduction to pure DP case. 
\cite{murtagh2016complexity} give a proof for non-interactive setting by conditioning on some special events and making reduction to pure DP case. 
The proof idea of our result is that for multi-round interactive protocol with maximal number of rounds $r$, we allow ourselves to condition on an event on every round. Specifically, for each round we pay a $\delta^{\frac{1}{r}}$ probability event. That corresponds to paying at most $r\delta^{\frac{1}{r}}$ probability to reduce to the case of pure differential privacy.

To prove the main result, we first set up some definitions and notations. We say $\mechanism$ is an \emph{$r$-round} interactive mechanism if for every adversary $\analyst$ it yields an $r$-round interactive protocol $(\analyst, \mechanism(\cdot))$. 

\begin{definition}
For a pair of adjacent datasets $x, x'$, an $r$-round interactive mechanism $\mechanism$ is $(\eps, \eps',\delta)$-differentially private on $(x, x')$ if for every adversary strategy $\analyst$ and every possible subset of views $T \subseteq \range(\view{\analyst}{\mechanism(\cdot)})$, we have:
\begin{equation} 
\Pr \left[\view{\analyst}{\mechanism(x)} \in T \right]
\leq e^{\eps}\cdot 
\Pr \left[\view{\analyst}{\mechanism(x')} \in T \right] + \delta \nonumber
\end{equation}
and
\begin{equation} 
\Pr \left[\view{\analyst}{\mechanism(x')} \in T \right]
\leq e^{\eps'}\cdot 
\Pr \left[\view{\analyst}{\mechanism(x)} \in T \right] + \delta \nonumber
\end{equation}
\end{definition}

\newcommand{\Ep}[1]{E_{p^{(#1)}}}
\newcommand{\qvec}[1]{\bm{q}^{(#1)}}
\newcommand{\msecond}{\mechanism^{>1}_{q_0, a_0}}
\newcommand{\msecondbrif}{\mechanism^{>1}}
\newcommand{\prefix}[1]{p^{(#1)}}

Given an adversary $\analyst$ and an interactive $\mechanism$, we say the \emph{transcript} in a session of interactive protocol $(\analyst, \mechanism(\cdot))$ as $t = (q_0, a_0, \ldots, q_{r-1}, a_{r-1})$. 
We further define the \emph{$i$th prefix of a transcript $t$} as $\prefix{i} = (q_0, a_0, \ldots, q_{i-2}, a_{i-2}, q_{i-1})$. We note that when $i=0$, $\prefix{0} = ()$ is an empty tuple. 
Without loss of generality, in the following theorem we assume the length of transcript for every $r$-round interactive protocol is exactly $2r$. If the protocol is terminated before $r$ rounds, we can simply fill in some dummy messages. 

\begin{theorem}
\label{thm:connection-approx}
For any pair of adjacent datasets $x, x'$, and for every $r$-round interactive mechanism $\mechanism$ that is $(\eps, \eps', \delta)$-differentially private on $(x, x')$, 
for every possible transcript between $(\analyst, \mechanism(\cdot))$, 
there is a collection of probabilistic events $\{\Ep{i}\}_{i=0}^{r}$, $\{\Ep{i}'\}_{i=0}^{r}$
defined over every possible prefix $\prefix{i}$ such that 
\begin{enumerate}
    \item The probability of the events $\Pr \left[\Ep{i} \right] = \Pr \left[\Ep{i}' \right] = 1-\delta^{1/r}$ every $0 \le i \le r$. 
    \item Summing the privacy losses conditioned on these events is at most $\eps$ and $\eps'$. That is, for every transcript $(q_0, a_0, \ldots, q_{r-1}, a_{r-1})$, 
    $$
    \sum_{i=1}^{r} \log \left( \frac{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]}{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]} \right) \le \eps
    $$
    and 
    $$
    \sum_{i=1}^{r} \log \left( \frac{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]}{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]} \right) \le \eps'
    $$
    (there are no privacy loss when $i=0$ by definition).
\end{enumerate}
\end{theorem}

\begin{proof}

We prove the statements of theorem by induction.

\paragraph{Base Case} 
When $r=0$, there are no privacy loss and therefore events $\Ep{0}$ and $\Ep{0}'$ trivially exists with probability 1 (by convention, $\delta^{\frac{1}{0}} = 0$ since $\delta<1$). 

%When $r=1$, $\mechanism$ is a non-interactive mechanism. Therefore, a natural generalization of Theorem \ref{thm:noninterac} to $(\eps_0, \eps_1, \delta)$ case shows that there are events $E_0^p, E_1^p$ with probability $1 - \delta$ s.t. 
%$$
%\log \left( \frac{\Pr[ A_1^0 = a_1 | E_0^{p_1} ]}{\Pr[ A_1^1 = a_1 | E_1^{p_1} ]} \right) \le \eps_0
%$$
%$$
%\log \left( \frac{\Pr[ A_1^1 = a_1 | E_1^{p_1} ]}{\Pr[ A_1^0 = a_1 | E_0^{p_1} ]} \right) \le \eps_1
%$$

\paragraph{Inductive Assumption} 
For every interactive mechanism $\mechanism$ that is $(\eps, \eps', \delta)$-differentially private mechanism on $(x, x')$ of total rounds $\le r-1$, 
for every possible transcript between $(\analyst, \mechanism(\cdot))$, 
there is a collection of probabilistic events $\left\{\Ep{i}\right\}_{i=0}^{r-1}$, $\left\{\Ep{i}'\right\}_{i=0}^{r-1}$
defined over every possible prefix $p^{(i)}$ such that 
\begin{enumerate}
    \item The probability of the events $\Pr \left[\Ep{i} \right] = \Pr \left[\Ep{i}' \right] = 1-\delta^{\frac{1}{r}}$ every $0 \le i \le r-1$. 
    \item Summing the privacy losses conditioned on these events is at most $\eps$ and $\eps'$, that is, 
    $$
    \sum_{i=1}^{r-1} \log \left( \frac{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]}{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]} \right) \le \eps
    $$
    and 
    $$
    \sum_{i=1}^{r-1} \log \left( \frac{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]}{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]} \right) \le \eps'
    $$
\end{enumerate}

\newcommand{\epssecond}{\eps_{>1}}


Before moving to the inductive step, we set up some notations first. In an interactive protocol $(\analyst, \mechanism(\cdot))$ where $\mechanism$ is an $r$-round interactive mechanism, given the first pair of query and response $(q_0, a_0)$, we can define an $(r-1)$-round interactive mechanism $\msecond$ that operates the same as $\mechanism$ for rounds $1, \ldots, r-1$ after receiving query $q_0$ and responding with $a_0$. That is, $\msecond(x_b)$ chooses coin tosses conditioned on the event $\mechanism(x_b, q_0)=a_0$. 
When $(q_0, a_0)$ is clear from the context, we simply write as $\msecondbrif$. 
Let $\delta^*=\delta^{1-\frac{1}{r}}$, we define $\epssecond(q_0,a_0)$ and $\epssecond'(q_0,a_0)$ as the minimum values s.t. $\msecondbrif$ is $(\epssecond(q_0,a_0), \epssecond'(q_0,a_0), \delta^*)$-differentially private on $(x, x')$.  

\paragraph{Inductive Step}
Given the first round transcript $(q_0, a_0)$, we can apply the inductive assumption to the $(r-1)$-round mechanism $\msecond$ which is 
$(\epssecond(q_0,a_0), \epssecond'(q_0,a_0), \delta^{1-\frac{1}{r}})$-differentially private on $(x, x')$. 
We denote the prefix for transcripts between $(\analyst, \msecondbrif(\cdot))$ as $\prefix{i}_{[1:]} = (q_1, a_1, \ldots, q_{i-1}, a_{i-1})$, and similarly $\qvec{i}_{[1:]} = (q_1, \ldots, q_{i-1})$. 
Given a transcript between $(\analyst, \mechanism(\cdot))$, for every prefix $\prefix{i}$ with $i \ge 1$ that begins with $(q_0, a_0)$ we can define events $\Ep{i}, \Ep{i}'$ the same as the events $E_{\prefix{i}_{[1:]}}, E_{\prefix{i}_{[1:]}}'$ for $\msecondbrif$. Therefore, we know that 
$\Pr \left[\Ep{i} \right] 
= \Pr \left[E_{\prefix{i}_{[1:]}} \right] 
= \Pr \left[\Ep{i} \right] 
= \Pr \left[E_{\prefix{i}_{[1:]}} \right] 
= 1-\delta^{(1-\frac{1}{r})\frac{1}{r-1}} 
= 1 - \delta^{\frac{1}{r}}$, and 
\begin{align}
&\sum_{i=1}^{r} \log \left( \frac{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]}{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]} \right) \nonumber \\
&=\sum_{i=2}^{r} \log \left( \frac{\Pr \left[ \msecondbrif(x, \qvec{i-1}_{[1:]}) = a_i | E_{\prefix{i-1}_{[1:]}} \right]}{\Pr \left[ \msecondbrif(x', \qvec{i-1}_{[1:]}) = a_i | E_{\prefix{i-1}_{[1:]}}' \right]} \right) \nonumber \\
&\le \epssecond(q_0,a_0) \nonumber
\end{align}
and
\begin{align}
&\sum_{i=2}^{r} \log \left( \frac{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]}{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]} \right) \nonumber \\
&=\sum_{i=2}^{r} \log \left( \frac{\Pr \left[ \msecondbrif(x', \qvec{i-1}_{[1:]}) = a_i | E_{\prefix{i-1}_{[1:]}}' \right]}{\Pr \left[ \msecondbrif(x, \qvec{i-1}_{[1:]}) = a_i | E_{\prefix{i-1}_{[1:]}} \right]} \right) \nonumber \\
&\le \epssecond'(q_0,a_0) \nonumber
\end{align}

It remains to show that we can construct events $E_{\prefix{1}}$ and $E'_{\prefix{1}}$ for every prefix $\prefix{1} = (q_0)$. To prove it, we need another observation. For readability, when $q_0$ is clear from the context, we drop it and denote the random variable of the first response $\mechanism(x, q_0)$ as $\mechanism(x)$. We also denote $\epssecond(q_0, a_0)$ as $\epssecond(a_0)$. 
We define the following disjoint sets:
$$
S = \{ a_0: \Pr[\mechanism(x)=a_0] > e^{\eps-\epssecond(a_0)} \Pr[\mechanism(x')=a_0] \}
$$
$$
T = \{ a_0: \Pr[\mechanism(x')=a_0] > e^{\eps'-\epssecond'(a_0)} \Pr[\mechanism(x)=a_0] \}
$$

Let 
$$
\alpha = \Pr[\mechanism(x) \in S] - e^{\eps-\epssecond(a_0)} \Pr[\mechanism(x') \in S] 
\ge 0
$$
$$
\beta = \Pr[\mechanism(x') \in T] - e^{\eps'-\epssecond'(a_0)} \Pr[\mechanism(x) \in T] \ge 0 $$

\newcommand{\ropt}{R^{OPT}}
\begin{claim}
Both $\alpha$ and $\beta$ are less than or equal to $\delta^{\frac{1}{r}}$. 
\end{claim}
\begin{proof}
By definition of $\epssecond$, given $(q_0, a_0)$ there is an adversary strategy $\analyst_{q_0, a_0}$ s.t. the bound $$
\Pr \left[\view{\analyst}{\msecond(x)} \in R \right] 
\le e^{\epssecond(q_0, a_0)}
\Pr \left[\view{\analyst}{\msecond(x')} \in R \right]  + \delta^{1-\frac{1}{r}}
$$
is tight for some set $R$. 
Let $\ropt_{q_0,a_0}$ denote the optimal distinguishing set $R$. 
Consider the adversary $\analyst$ which makes the first query $q_0$, and if get response $a_0 \in S$, uses the $(r-1)$-round strategy $\analyst_{q_0,a_0}$ with $\analyst$'s randomness $r$. 
Now, define $\ropt = \{(a_0,\ldots,a_{r-1}): a_0 \in S \wedge (r, a_1,\ldots,a_{r-1})\in \ropt_{q_0, a_0}\}$.

Define 
$$\Delta(a_0) = \Pr[\mechanism(x)=a_0]-
e^{\eps-\epssecond(a_0)}\cdot\Pr[\mechanism(x')=a_0]$$
Observe that 
\begin{align}
\sum_{a_0 \in S} \Delta(a_0)
&= \sum_{a_0 \in S} \Pr[\mechanism(x)=a_0]-
e^{\eps-\epssecond(a_0)}\cdot \sum_{a_0 \in S}\Pr[\mechanism(x')=a_0] \nonumber \\
&= \Pr[\mechanism(x) \in S] - e^{\eps-\epssecond(a_0)} \Pr[\mechanism(x') \in S] \nonumber \\
&= \alpha \nonumber
\end{align}


For adversary $\analyst$, we have 
\begin{equation}
\begin{split}
&\Pr[\view{\analyst}{\mechanism(x)} \in \ropt]\\
&= \sum_{a_0 \in S} 
\Pr[\mechanism(x_0)=a_0] 
\Pr[\view{\analyst_{q_0, a_0}}{\msecond(x)} \in \ropt_{q_0, a_0}] \\
&= 
\sum_{a_0 \in S} \left(e^{\eps-\epssecond(a_0)}\cdot\Pr[\mechanism(x')=a_0]+\Delta(a_0) \right) \left( e^{\epssecond(q_0, a_0)} \Pr \left[\view{\analyst}{\msecond(x')} \in \ropt_{q_0, a_0} \right]  + \delta^{1-\frac{1}{r}} \right) \\
&\ge e^{\eps} \cdot \Pr \left[\view{\analyst}{\mechanism(x')} \in \ropt \right] + \alpha \delta^{1-\frac{1}{r}}  \nonumber
\end{split}
\end{equation}
Since $\mechanism$ is $(\eps, \eps', \delta)$-differentially private on $(x, x')$, we must have $\alpha \delta^{1-\frac{1}{r}} \le \delta$, which means that $\alpha \le \delta^{\frac{1}{r}}$. 

By a symmetric argument, we can also show that $\beta \le \delta^{\frac{1}{r}}$.  
\end{proof}

We are ready to construct the events for prefixes with length 1 now. 
\begin{claim}
For every prefix $\prefix{1} = (q_0)$, there are events $E  = E_{\prefix{1}}$ and $E' = E_{\prefix{1}}'$ each with probability $1-\delta^{\frac{1}{r}}$, and for every possible response $a_0$, we have 
$$ 
\log \left( \frac{\Pr \left[\mechanism(x,q_0)=a_0|E \right]}{\Pr \left[\mechanism(x',q_0)=a_0|E' \right]} \right) 
\leq \eps - \epssecond(q_0,a_0)
$$
$$ 
\log \left( \frac{\Pr \left[\mechanism(x',q_0)=a_0|E' \right]}{\Pr \left[\mechanism(x,q_0)=a_0|E \right]} \right) 
\leq \eps' - \epssecond'(q_0,a_0)
$$
\end{claim}


\begin{proof}

This proof follows the construction of \cite{murtagh2016complexity}. Finding events $E$, $E'$ with probability $1-\delta^{\frac{1}{r}}$ is equivalent to find functions $e, f$ s.t. 
\begin{enumerate}
    \item For all $a_0$, $0 \le e(a_0) \le \Pr[\mechanism(x)=a_0]$, $0 \le f(a_0) \le \Pr[\mechanism(x')=a_0]$
    \item For all $a_0$, $e(a_0) \le e^{\eps - \epssecond(a_0)} f(a_0)$, $f(a_0) \le e^{\eps' - \epssecond'(a_0)} e(a_0)$
    \item $\sum_{a_0} e(a_0) = 1-\delta^{\frac{1}{r}}$, $\sum_{a_0} f(a_0) = 1-\delta^{\frac{1}{r}}$.
\end{enumerate}
Indeed, the corresponding events are then defined by 
$$
\Pr \left[E | \mechanism(x)=a_0 \right] = \frac{e(a_0)}{\Pr[\mechanism(x)=a_0]}
$$
$$
\Pr[E' | \mechanism(x')=a_0] = \frac{f(a_0)}{\Pr[\mechanism(x')=a_0]}
$$
By Bayes' Rule, the conditions above imply that 
\begin{align}
\Pr[\mechanism(x)=a_0 | E ] 
&= \frac{ \Pr[E | \mechanism(x)=a_0] \Pr[\mechanism(x)=a_0] }{ \Pr[E] } \nonumber \\
&= \frac{e(a_0)}{\sum_y e(y)} \nonumber \\
&\le \frac{ e^{\epszero - \epszerogo} f(a_0) }{ \sum_y f(y) } \nonumber \\
&= e^{\epszero - \epszerogo} \Pr \left[ \mechanism(x')=a_0 | E' \right] \nonumber
\end{align}


Now, we start to define functions $e, f$ as the following:
\begin{enumerate}
    \item For $a_0 \in S, e(a_0)=e^{\eps - \epssecond(a_0)} \cdot \operatorname{Pr}[\mechanism(x')=a_0]$ and for $a_0 \notin S, e(a_0)=\operatorname{Pr}[\mechanism(x) =a_0]$. 
    \item For $a_0 \in T, f(a_0)=e^{\eps' - \epssecond'(a_0)} \cdot \operatorname{Pr}[\mechanism(x) =a_0]$ and for $a_0 \notin T, f(a_0)=\operatorname{Pr}[\mechanism(x') =a_0]$
\end{enumerate}

Since $\alpha \le \delta^{\frac{1}{r}}$ and $\beta \le \delta^{\frac{1}{r}}$, 
we have $\sum_{a_0} e(a_0) = 1-\alpha \ge 1-\delta^{\frac{1}{r}}$, $\sum_{a_0} f(a_0) = 1-\beta \ge 1-\delta^{\frac{1}{r}}$. 
The only remaining work is to modify $e, f$ with $\sum_{a_0} e(a_0) = 1-\delta^{\frac{1}{r}}$, $\sum_{a_0} f(a_0) = 1-\delta^{\frac{1}{r}}$ by making $\alpha=\beta=\delta^{\frac{1}{r}}$. 
We will first modify $e$ and $f$ so that $\alpha = \beta$, and then decrease $e, f$ so that $\alpha = \beta = \delta^{\frac{1}{r}}$. 
Suppose, without loss of generality that $\alpha > \beta$, then we will reduce the function $f$ on the set $T' = \{a_0: \Pr[\mechanism(x')=a_0] > \Pr[\mechanism(x)=a_0] \}$ in order to reduce the sum $\sum_{a_0} f(a_0)$ by $\alpha - \beta$, where we know that $T \subseteq T'$, while maintaining all the other conditions. The only condition that might be violated if we reduce the function $f$ is the one that $e(a_0) \le e^{\eps - \epssecond(a_0)} f(a_0)$. So we just need to confirm that 
$$
\sum_{a_0 \in T'} (f(a_0) - e^{\epssecond(a_0)-\eps} \cdot e(a_0))
$$
is at least $\alpha - \beta$ to be able to reduce $f$ as much as we need. Since we have 
$$
\sum_{a_0 \in T'} (f(a_0) - e^{\epssecond(a_0)-\eps} \cdot e(a_0)) \ge 
\sum_{a_0 \in T'} (f(a_0) - e(a_0))
$$
so it suffices to show that the area of the region that is above $e(a_0)$ and below $f(a_0)$ is at least $\alpha - \beta$. To see this, we make the following observations.
\begin{enumerate}
    \item The area of the region that is above $\Pr[\mechanism(x) = a_0]$ and below $\Pr[\mechanism(x') = a_0]$ is equal to the region that is above $\Pr[\mechanism(x') = a_0]$ and below $\Pr[\mechanism(x) = a_0]$ (it is just the total variation distance between them). 
    \item The area of the region that is above $\Pr[\mechanism(x) = a_0]$ and below $\Pr[\mechanism(x') = a_0]$ equals $\beta$ plus the area of the region that is above $e(a_0)$ and below $f(a_0)$. 
    \item The area of the region that is above $\Pr[\mechanism(x') = a_0]$ and below $\Pr[\mechanism(x) = a_0]$ is at least $\alpha$. 
\end{enumerate}
Putting it all together, we have 
\begin{align}
    &\sum_{a_0 \in T'} (f(a_0) - e^{-\eps} \cdot e(a_0)) \nonumber \\
    &\ge \sum_{a_0 \in T'} (f(a_0) - e(a_0)) \nonumber \\
    &= \sum_{a_0 \in T'} (\Pr[\mechanism(x') = a_0] - \Pr[\mechanism(x) = a_0]) - \beta \nonumber \\
    &\ge \alpha - \beta \nonumber
\end{align}
Therefore, we can reduce $\sum_{a_0}f(a_0)$ by $\alpha - \beta$ without violating the other conditions and thus get two new functions $e$ and $f$ such that 
\begin{enumerate}
    \item For all $a_0$, $0 \le e(a_0) \le \Pr[\mechanism(x)=a_0]$, $0 \le f(a_0) \le \Pr[\mechanism(x')=a_0]$
    \item For all $a_0$, $e(a_0) \le e^{\eps - \epssecond(a_0)} f(a_0)$, $f(a_0) \le e^{\eps' - \epssecond'(a_0)} e(a_0)$
    \item $\sum_{a_0} e(a_0) = \sum_{a_0} f(a_0) \ge 1-\delta^{\frac{1}{r}}$.
\end{enumerate}
Suppose $\sum_{a_0} e(a_0)= \sum_{a_0} f(a_0) = 1-\delta_0 > 1-\delta^{\frac{1}{r}}$, then we can scale them both by a multiplicative factor of $\frac{1-\delta_0}{1-\delta^{\frac{1}{r}}}$ and achieve all the desired conditions. 
 

%\begin{figure}[H]
%    \centering%
%	\includegraphics[width=0.5\textwidth]{images/proof-illustration.png}
%\end{figure} 

\end{proof}

We thus complete the induction argument and are able to show the second statement in the theorem. 
\begin{align}
&\sum_{i=1}^{r} \log \left( \frac{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]}{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]} \right) \nonumber \\
& = \log \left( \frac{\Pr \left[ \mechanism(x, \qvec{1}) = a_0 | \Ep{0} \right]}{\Pr \left[ \mechanism(x', \qvec{1}) = a_0 | \Ep{0}' \right]} \right) + 
\sum_{i=1}^{r-1} \log \left( \frac{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]}{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]} \right) \nonumber \\
&\le \eps-\epssecond(a_0) + \epssecond(a_0) = \eps \nonumber
\end{align}
and symmetrically we have 
\begin{align}
&\sum_{i=1}^{r} \log \left( \frac{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]}{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]} \right) \nonumber \\
& = \log \left( \frac{\Pr \left[ \mechanism(x', \qvec{1}) = a_0 | \Ep{0}' \right]}{\Pr \left[ \mechanism(x, \qvec{1}) = a_0 | \Ep{0} \right]} \right) + 
\sum_{i=1}^{r-1} \log \left( \frac{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]}{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]} \right) \nonumber \\
&\le \eps'-\epssecond'(a_0) + \epssecond'(a_0) = \eps' \nonumber
\end{align}
\end{proof}

\begin{remark}
Two parts are discarded in Inequality 29:
$$
\delta^{1-\frac{1}{r}} \sum_{a_1 \in S} e^{\eps_0-\eps_0^{>1}(q_1, a_1)}\cdot\Pr[M(x_1,q_1)=a_1]
$$ and 
$$
\sum_{a_1 \in S} \Delta(a_1) e^{\eps_0^{>1}(q_1, a_1)} \Pr[\View(\analystq \leftrightarrow \mechq{a_1}(x_1)) \in S_{q_1, a_1}]
$$
\end{remark}

Following the above results, we immediately have the following theorem. 
\begin{theorem}
\label{thm:reduce-noninteractive}
Suppose that $\mechanism$ is an $r$-round interactive $(\eps, \delta)$-differentially private mechanism. Then for every pair of adjacent datasets $x_0, x_1$, there is an interactive mechanism $T$ s.t. for every adversary $\analyst$ and every $b \in \{0, 1\}$ we have 
\begin{equation}
\view{\analyst}{\mechanism(x_b)} 
\equiv 
\view{\analyst}{T(\RR_{ \left( \varepsilon, 0 \right)}(b))} \nonumber
\end{equation}
\end{theorem}
\begin{proof}
By Theorem \ref{thm:connection-approx}, we know that for any possible transcript in a protocol $(\analyst, \mechanism(\cdot))$, there is a collection of probabilistic events 
%$E = \left\{E_{p^{(i)}}\right\}_{i=0}^{r-1}$, $E' = \left\{E'_{p^{(i)}}\right\}_{i=0}^{r-1}$ 
$E = \bigcup_{i=0}^{r-1} E_{p^{(i)}}$, $E' = \bigcup_{i=0}^{r-1} E'_{p^{(i)}}$ 
s.t. 
$$
\sum_{i=0}^{r-1} \log \left( \frac{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]}{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]} \right) \le \eps
$$
and 
$$
\sum_{i=0}^{r-1} \log \left( \frac{\Pr \left[ \mechanism(x', \qvec{i}) = a_i | \Ep{i}' \right]}{\Pr \left[ \mechanism(x, \qvec{i}) = a_i | \Ep{i} \right]} \right) \le \eps
$$
and $\Pr[E] = \Pr[E'] \ge 1-r\delta^{\frac{1}{r}}$ by union bound. 
Thus, we can define a dummy event $H$ that is independent of everything else and
$\Pr[ H ]= (1-r\delta^{\frac{1}{r}})/\Pr[E]$. Particularly, the output distribution of $\mechanism$ is independent of $H$. 


We construct the simulating mechanism $T$ as follows: 

\begin{enumerate}
    \item If $t=0$, we have
    \begin{align}
    \Pr \left[ T(0, q_0)=a_0 \right] 
    %&= \frac{ e^\eps \Pr[\mechanism(x_0, q_0)=a_0 | E_{p^{(0)}} \wedge H ] - \Pr[\mechanism(x_1, q_0)=a_0 | E'_{p^{(0)}} \wedge H] }{e^\eps - 1} \nonumber \\
    &= \frac{ e^\eps \Pr[\mechanism(x_0, q_0)=a_0 | E_{p^{(0)}} ] - \Pr[\mechanism(x_1, q_0)=a_0 | E'_{p^{(0)}}] }{e^\eps - 1} \nonumber
    \end{align}
    \begin{align}
    \Pr \left[ T(1, q_0)=a_0 \right] 
    %&= \frac{ e^\eps \Pr[\mechanism(x_1, q_0)=a_0 | E'_{p^{(0)}} \wedge H ] - \Pr[\mechanism(x_0, q_0)=a_0 | E_{p^{(0)}} \wedge H] }{e^\eps - 1} \nonumber \\
    &= \frac{ e^\eps \Pr[\mechanism(x_1, q_0)=a_0 | E'_{p^{(0)}} ] - \Pr[\mechanism(x_0, q_0)=a_0 | E_{p^{(0)}}] }{e^\eps - 1} \nonumber
    \end{align}
    \begin{align}
    \Pr \left[ T(\iamzero, q_0)=a_0 \right] 
    %&=  \Pr \left[\mechanism(x_0, q_0)=a_0 | \neg ( E_{p^{(0)}} \wedge H) \right] \nonumber \\
    &= \Pr \left[\mechanism(x_0, q_0)=a_0 | \neg E_{p^{(0)}} \right] \nonumber \nonumber
    \end{align}
    \begin{align}
    \Pr \left[ T(\iamone, q_0)=a_0 \right] 
    %&=  \Pr \left[\mechanism(x_1, q_0)=a_0 | \neg ( E_{p^{(0)}}' \wedge H) \right] \nonumber \\
    &= \Pr \left[\mechanism(x_1, q_0)=a_0 | \neg E_{p^{(0)}}' \right] \nonumber \nonumber
    \end{align}
    
    \item If $t>0$, given earlier responses $(a_0, \dots, a_{t-2})$, we define 
    \begin{align}
    &\Pr \left[ T(0, \bm{q}^{(t)}) = a_{t-1} | a_0, \dots, a_{t-2} \right] \nonumber \\
    &= \frac{e^\eps \Pr \left[ \vec{\mechanism}(x_0, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) | \bigcup_{i=0}^{t-1} E_{p^{(i)}} \right] - \Pr \left[ \vec{\mechanism}(x_1, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) | \bigcup_{i=0}^{t-1} E'_{p^{(i)}} \right] }{(e^\eps - 1) \Pr \left[ \vec{T}(0, \bm{q}^{(t-1)}) = (a_0, \dots, a_{t-2}) \right] } \nonumber
    \end{align}
    \begin{align}
    &\Pr \left[ T(1, \bm{q}^{(t)}) = a_{t-1} | a_0, \dots, a_{t-2} \right] \nonumber \\
    &= \frac{e^\eps \Pr \left[ \vec{\mechanism}(x_1, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) | \bigcup_{i=0}^{t-1} E'_{p^{(i)}} \right] - \Pr \left[ \vec{\mechanism}(x_0, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) | \bigcup_{i=0}^{t-1} E_{p^{(i)}} \right] }{(e^\eps - 1) \Pr \left[ \vec{T}(1, \bm{q}^{(t-1)}) = (a_0, \dots, a_{t-2}) \right] } \nonumber
    \end{align}
    \begin{align}
    \Pr \left[ T(\iamzero, \bm{q}^{(t)}) = a_{t-1} | a_0, \dots, a_{t-2} \right] \nonumber = \Pr \left[ \vec{\mechanism}(x_0, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) |  \neg \bigcup_{i=0}^{t-1} E_{p^{(i)}} \right] \nonumber
    \end{align}
    \begin{align}
    \Pr \left[ T(\iamone, \bm{q}^{(t)}) = a_{t-1} | a_0, \dots, a_{t-2} \right] \nonumber = \Pr \left[ \vec{\mechanism}(x_1, \bm{q}^{(t)})=(a_0, \dots, a_{t-1}) |  \neg \bigcup_{i=0}^{t-1} E'_{p^{(i)}} \right] \nonumber
    \end{align}
\end{enumerate}
We can easily verify that all of the above are valid probability distributions. Therefore, the distribution of $\vec{T}$ given a sequence of queries $\bm{q}^{(t)}$ is 
\begin{align}
    &\Pr \left[ \vec{T}(0, \bm{q}^{(t)}) = \at \right] \nonumber \\
    &= \frac{e^\eps \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | E \right] - \Pr \left[\vec{\mechanism}(x', \bm{q}^{(t)})=\at | E'\right] }{e^\eps - 1} \nonumber \\
    &= \frac{e^\eps \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | E \wedge H \right] - \Pr \left[\vec{\mechanism}(x', \bm{q}^{(t)})=\at | E' \wedge H \right] }{e^\eps - 1} \nonumber
\end{align}
\begin{align}
    &\Pr \left[ \vec{T}(1, \bm{q}^{(t)}) = \at \right] \nonumber \\
    &= \frac{e^\eps \Pr \left[\vec{\mechanism}(x', \bm{q}^{(t)})=\at | E' \right] - \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | E \right] }{e^\eps - 1} \nonumber \\
    &= \frac{e^\eps \Pr \left[\vec{\mechanism}(x', \bm{q}^{(t)})=\at | E' \wedge H \right] - \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | E \wedge H \right] }{e^\eps - 1} \nonumber
\end{align}
\begin{align}
    \Pr \left[ \vec{T}(\iamzero, \bm{q}^{(t)}) = \at \right]  
    &= \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | \neg E \right] \nonumber \\
    &= \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | \neg (E \wedge H) \right] \nonumber
\end{align}
\begin{align}
    \Pr \left[ \vec{T}(\iamone, \bm{q}^{(t)}) = \at \right] 
    &= \Pr \left[\vec{\mechanism}(x', \bm{q}^{(t)})=\at | \neg E' \right]  \nonumber \\
    &= \Pr \left[\vec{\mechanism}(x', \bm{q}^{(t)})=\at | \neg (E' \wedge H) \right]  \nonumber 
\end{align}

% Let $\newdelta = \newdelta$. 
Thus, the output distribution of $T$ with the input $\RR_{\left(\eps, 0 \right)}(0)$ as computed as
\begin{align}
&\Pr \left[T \left(\RR_{\left(\eps, 0 \right)}(0) \right) = \at \right] \nonumber \\
&= \newdelta \cdot \Pr[T(\iamzero) = \at] 
+ \frac{(1-\newdelta)e^{\eps}}{1+e^\eps} \cdot \Pr[T(0) = \at] + \frac{(1-\newdelta)}{1+e^\eps} \cdot \Pr[T(1) = \at] + 0 \nonumber \\
&= \newdelta \cdot \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | \neg E \right] \nonumber \\
&~~~+ \frac{(1-\newdelta)e^{\eps}}{1+e^\eps} \cdot \frac{e^\eps \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | E \right] - \Pr \left[\vec{\mechanism}(x', \bm{q}^{(t)})=\at | E' \right] }{e^\eps - 1} \nonumber \\
&~~~+ \frac{(1-\newdelta)}{1+e^\eps} \cdot \frac{e^\eps \Pr \left[\vec{\mechanism}(x', \bm{q}^{(t)})=\at | E' \right] - \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | E \right] }{e^\eps - 1} \nonumber \\
&= \newdelta \cdot \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | \neg E \right] 
+ (1-\newdelta) \cdot \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | E \right] \nonumber \\
&= \Pr[\neg (E \wedge H)] \cdot \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | \neg (E \wedge H) \right]  + 
\Pr[E \wedge H] \cdot \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at | E \wedge H \right] \nonumber \\
&= \Pr \left[\vec{\mechanism}(x, \bm{q}^{(t)})=\at \right] \nonumber
\end{align}
The case when the input of $\RR$ is 1 could be similarly proved. Therefore, we proved the existence of such an interactive mechanism $T$ for any $(\eps, \delta)$ interactive DP mechanisms. 
\end{proof}
\end{comment}

\newcommand{\concomppriv}{\mathrm{OptCompPriv}}

The above theorem suggests that the non-interactive $\RR_{\left(\varepsilon, 0 \right)}$ can simulate any $(\eps, 0)$ interactive DP algorithm. Since it is known that post-processing preserves differential privacy (Theorem \ref{thm:post-processing}), it follows that to analyze the concurrent composition of arbitrary $(\eps_i, 0)$ interactive differentially private algorithms, it suffices to analyze the composition of randomized response $\RR_{\left(\eps_i, 0 \right)}$. 
For interactive mechanisms $\mechanism_0, \ldots, \mechanism_{k-1}$ and a given target confidence parameter $\delta_g$, we use $\concomppriv(\mechanism_0, \ldots, \mechanism_{k-1}; \delta_g)$ to denote the privacy parameter $\eps_g$ of the concurrent composition $\concomp(\mechanism_0, \ldots, \mechanism_{k-1})$. 
That is, 
\begin{align}
&\concomppriv(\mechanism_0, \ldots, \mechanism_{k-1}; \delta_g) \nonumber \\
&= \inf \left\{\varepsilon_{g} \geq 0: \concomp(\mechanism_{0}, \ldots, \mechanism_{k-1}) \text { is }\left(\varepsilon_{g}, \delta_{g}\right)\mathrm{-DP}\right\} \nonumber
\end{align}

\begin{lemma} 
Suppose there are interactive mechanisms $\mechanism_0, \ldots, \mechanism_{k-1}$ where for each $0 \le i \le k-1$, $\mechanism_i$ is $(\eps_i, 0)$-differentially private. For any values of $\eps_0, \dots, \eps_{k-1} \ge 0$, $\delta_g \in [0, 1)$, we have
\begin{align}
&\concomppriv( \mechanism_0, \ldots, \mechanism_{k-1}, \delta_g) \nonumber \\
&= \concomppriv \left(\RR_{(\eps_0, 0)}, \dots, \RR_{(\eps_{k-1}, 0)}, \delta_g \right) \nonumber
\end{align}
\end{lemma}
\begin{proof}
We want to show that 
\begin{align}
&\inf \left\{\varepsilon_{g} \geq 0: \concomp(\mechanism_{0}, \ldots, \mechanism_{k-1}) \text { is }\left(\varepsilon_{g}, \delta_{g}\right)\mathrm{-DP}\right\} \nonumber \\
&= \inf \left\{\varepsilon_{g} \geq 0: \concomp \left(\RR_{(\eps_0, 0)}, \dots, \RR_{(\eps_{k-1}, 0)} \right) \text { is }\left(\varepsilon_{g}, \delta_{g}\right)\mathrm{-DP}\right\} \nonumber
\end{align}


Since the non-interactive $\RR_{(\eps_0, 0)}, \dots, \RR_{(\eps_{k-1}, 0)}$ can be viewed as a special case of interactive DP mechanisms, we have 
\begin{align}
&\inf \left\{\varepsilon_{g} \geq 0: \concomp(\mechanism_{0}, \ldots, \mechanism_{k-1}) \text { is }\left(\varepsilon_{g}, \delta_{g}\right)\mathrm{-DP}\right\} \nonumber \\
&\ge \inf \left\{\varepsilon_{g} \geq 0: \concomp \left(\RR_{(\eps_0, 0)}, \dots, \RR_{(\eps_{k-1}, 0)} \right) \text { is }\left(\varepsilon_{g}, \delta_{g}\right)\mathrm{-DP}\right\} \nonumber
\end{align}

For the other direction, suppose $\concomp \left(\RR_{(\eps_0, 0)}, \dots, \RR_{(\eps_{k-1}, 0)} \right)$ is $(\eps_g^*, \delta_g)$-DP. We will show that $\concomp(\mechanism_0, \ldots, \mechanism_{k-1})$ is also $(\eps_g^*, \delta_g)$-DP. Taking the infimum over $\eps_g^*$ will then complete the proof. 

We know from Theorem \ref{thm:reduction-pure} that for every pair of adjacent datasets $x_0, x_1$, there must exist interactive mechanisms $T_0, \ldots, T_{k-1}$ such that for every adversary $\analyst$, $\view{\analyst}{\mechanism_i(x_b)}$ is identically distributed as $\view{\analyst}{T_i(\RR_{ \left( \varepsilon, 0 \right)}(b))}$ for all $i = 0, \ldots, k-1$. By hypothesis, we know that 
$\concomp \left(\RR_{(\eps_0, 0)}, \dots, \RR_{(\eps_{k-1}, 0)} \right)$ is $(\eps_g^*, \delta_g)$-differentially private, thus by post-processing inequality (Theorem \ref{thm:post-processing}) we know that 
\begin{align}
&\inf \left\{\varepsilon_{g} \geq 0: \concomp(\mechanism_{0}, \ldots, \mechanism_{k-1}) \text { is }\left(\varepsilon_{g}, \delta_{g}\right)\mathrm{-DP}\right\} \nonumber \\
&= \inf \left\{\varepsilon_{g} \geq 0: \concomp \left(T_0 \left(\RR_{(\eps_0, 0)} \right), \right. \right. \\
&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\dots, \\
&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\left. \left. T_{k-1} \left(\RR_{(\eps_{k-1}, 0)} \right) \right) \text { is }\left(\varepsilon_{g}, \delta_{g}\right)\mathrm{-DP}\right\} \nonumber \\
&\le \inf \left\{\varepsilon_{g} \geq 0: \concomp \left(\RR_{(\eps_0, 0)}, \RR_{(\eps_{k-1}, 0)} \right) \text { is }\left(\varepsilon_{g}, \delta_{g}\right)\mathrm{-DP}\right\} \nonumber \\
&\le \eps_g^* \nonumber
\end{align}
\end{proof}

We note that $\RR_{(\eps_0, 0)}, \dots, \RR_{(\eps_{k-1}, 0)}$ are non-interactive mechanisms, therefore we can use any composition theorems for non-interactive DP mechanisms to bound the privacy parameter of their composition. The tightest composition theorem for non-interactive DP is derived in \cite{murtagh2016complexity}. 

\begin{theorem}[Optimal Composition Theorem for Non-interactive DP]
If $\mechanism_0, \dots, \mechanism_{k-1}$ are each $(\eps_i, \delta_i)$-differentially private, then given the target security parameter $\delta_g$, the privacy parameter of concurrent composition $\concomp(\mechanism_0, \dots, \mechanism_{k-1})$ is
upper bounded by the least value of $\varepsilon_{g} \geq 0$ such that
$$
\frac{1}{\prod_{i=0}^{k-1}\left(1+\mathrm{e}^{\varepsilon_{i}}\right)} 
\sum_{S \subseteq\{0, \ldots, k-1\}} \max 
\left
\{\mathrm{e}^{\sum_{i \in S} \varepsilon_{i}}-\mathrm{e}^{\varepsilon_{g}} \cdot \mathrm{e}^{\sum_{i \notin S} \varepsilon_{i}}, 0
\right\} 
\leq 1-\frac{1-\delta_{g}}{\prod_{i=0}^{k-1}\left(1-
\delta_{i} \right)}
$$
\end{theorem}
Therefore, we are ready to bound the concurrent composition for an arbitrary set of interactive differentially private algorithms by simply plugging parameters to the optimal composition bound for non-interactive DP mechanisms in \cite{murtagh2016complexity}. 

\reducenonint*

\begin{comment}
\begin{theorem}[Optimal Composition Theorem for Pure Non-interactive DP]
If $\mechanism_0, \dots, \mechanism_{k-1}$ are each $(\eps_i, 0)$-differentially private, then given the target security parameter $\delta_g$, the privacy parameter of concurrent composition $\concomp(\mechanism_0, \dots, \mechanism_{k-1})$ is
upper bounded by the least value of $\varepsilon_{g} \geq 0$ such that
$$
\frac{1}{\prod_{i=0}^{k-1}\left(1+\mathrm{e}^{\varepsilon_{i}}\right)} 
\sum_{S \subseteq\{0, \ldots, k-1\}} \max 
\left
\{\mathrm{e}^{\sum_{i \in S} \varepsilon_{i}}-\mathrm{e}^{\varepsilon_{g}} \cdot \mathrm{e}^{\sum_{i \notin S} \varepsilon_{i}}, 0
\right\} 
\leq \delta_g
$$
\end{theorem}
\end{comment}

==> experiment.tex <==

The plots in Figure \ref{fig:varyeps}, Figure \ref{fig:varydeltag} compare the performances of the Theorem \ref{thm:concomp-basic-approx} and Theorem \ref{thm:bound-opt} in homogeneous case. 
In all figures, ``GroupPriv'' refers to the bound in Theorem \ref{thm:concomp-basic-approx} (since it reduces to the same bound as group privacy for homogeneous setting), ``RandomResp'' refers to the bound in Theorem \ref{thm:bound-opt} (since it is essentially the optimal composition of randomized response). 
Here we are composing $k$ mechanisms that are $(\eps, 0)$ differentially private to obtain an $(\eps_g, \delta_g)$ differentially private interactive mechanisms as guaranteed by one of the composition theorems. 

\begin{comment}
Note that Theorem \ref{thm:concomp-basic-approx} outputs both $(\eps_g, \delta_g)$, therefore we use the following theorem to adjust the tradeoff between $\eps_g$ and $\delta_g$.  

\begin{theorem}[Tightest tradeoff between $\eps$ and $\delta$ for $(\eps, \delta)$-DP \cite{cuff2016differential}]
\label{thm:tradeoff}
For any $1 > \delta' > \delta > 1$, let $\eps' = \ln( \frac{ (1-\delta')(e^{\eps}+1) }{1-\delta} - 1 )$, then 
$$
P \approx_{(\eps, \delta)} Q \implies 
P \approx_{(\eps', \delta')} Q
$$
\end{theorem}
%\begin{proof}
%Easily adapt from \url{https://arxiv.org/pdf/1608.03677.pdf} Appendix B. 
%\end{proof}
\end{comment}

\begin{figure}[H]
    \centering
	\subfigure[]{
	\includegraphics[width=0.45\columnwidth]{images/vary_eps_k700.png}
	}
	\subfigure[]{
	\includegraphics[width=0.45\columnwidth]{images/vary_eps_k100.png}
	}
	\caption{$\eps_g$ given by the three composition theorems for varying values of $\eps$ as $k$ grows. Parameters are $\delta=0$, $\delta_g=10^{-5}$. The figure on the right zoomed in on the $k<100$ regime. We can see that Theorem \ref{thm:bound-opt} gives substantial savings in $\eps_g$ even for moderate values of $k$. }
	\label{fig:varyeps}
\end{figure}

\begin{figure}[H]
    \centering
	\subfigure[]{
	\includegraphics[width=0.45\columnwidth]{images/vary_gdelta.png}
	}
	\caption{$\eps_g$ given by the three composition theorems for varying values of $\delta_g$ as $k$ grows. Parameters are $\delta=0$, $\eps=0.005$. $\delta_g$ does not affect $\eps_g$ in Theorem \ref{thm:concomp-basic-approx}. }
	\label{fig:varydeltag}
\end{figure}

\begin{comment}
\begin{figure}[H]
	\subfigure[]{
	\includegraphics[width=0.45\columnwidth]{images/vary_R.png}
	}
	\subfigure[]{
	\includegraphics[width=0.45\columnwidth]{images/vary_R_float.png}
	}
	\caption{(Left) $\eps_g$ given by the three composition theorems for varying values of $r$ as $k$ grows. Parameters are $\delta=10^{-128}$, $\eps=0.005$ and $\delta_g=10^{-5}$. $r$ does not affect $\eps_g$ in Theorem \ref{thm:concomp-basic-approx}. We can see that $r$ will only affect $\eps_g$ obtained from Theorem \ref{thm:bound-opt} when $k$ is very large. (Right) $\eps_g$ given by the three composition theorems for varying values of $\delta$ as $r$ grows. Parameters are $\eps=0.005$, $k=5$ and $\delta_g = 10^{-5}$. We can see that although Theorem \ref{thm:bound-opt} only applies when $r$ is small, it gives substantial savings in $\eps_g$ even for the largest $r$ it can use. }
	\label{fig:varyR}
\end{figure}
\end{comment}


==> intro.tex <==
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\MS}{\mathrm{MultiSets}}

Differential privacy is a framework for protecting privacy when performing statistical
releases on a dataset with sensitive information about individuals.  
%that allows statistical analysis of private databases while minimizing the risks to individuals in the databases. 
Specifically, for a differentially private mechanism, the probability distribution of the mechanism's outputs of a dataset should be nearly identical to the distribution of its outputs on the same dataset with any single individual’s data replaced. To formalize this, we call two datasets $x$, $x'$, each multisets over a data universe $\cX$, {\em adjacent} if one can be obtained from the other by adding or removing a single element of $\cX$.
%with $n$ rows each \emph{adjacent} if they are identical on at least $n-1$ rows, and differential privacy is defined as follows.

\begin{definition}[Differential Privacy \citep{dwork2006calibrating}]
For $\eps, \delta \ge 0$, a randomized algorithm $\mechanism : \MS(\cX)\rightarrow \cY$ is 
{\em $(\eps, \delta)$-differentially private} if for every pair of adjacent datasets $x, x'\in \MS(\cX)$ and all sets $T \subseteq \cY$, we have: 
$$
\Pr[\mechanism(x) \in T] \le e^\eps\cdot \Pr[\mechanism(x') \in T] + \delta
$$
where the randomness is over the coin flips of the algorithm $\mechanism$. 
\end{definition}

In the practice of differential privacy, we generally view $\eps$ as ``privacy-loss budget'' that is small but non-negligible (e.g. $\eps=0.1$), and we view $\delta$ as cryptographically negligible (e.g. $\delta=2^{-60}$). We refer to the case where $\delta=0$ as \emph{pure differential privacy}, and the case where $\delta >0$ as \emph{approximate differential privacy}. 

\salil{removed post-processing thm from intro, so insert it back into technical sections where it is needed}
\iffalse
One of the central properties of differential privacy is that it is preserved under ``post-processing'' \citep{dwork2006calibrating, dwork2014algorithmic}, which is formulated as follows:
\begin{theorem}[Post-processing]
\label{thm:post-processing}
If a randomized algorithm $\mechanism: \X \rightarrow \Y$ is $(\eps, \delta)$-differentially private, and $\mathcal{F}: \Y \rightarrow \mathcal{Z}$ is any randomized function, then $\mathcal{F} \circ \mechanism: \X \rightarrow \mathcal{Z}$ is also $(\eps, \delta)$-differentially private. 
\end{theorem}
\fi


Another important property of differential privacy is its behavior under composition. If we run multiple distinct differentially private algorithms on the same dataset, the resulting composed algorithm is also differentially private, with some degradation in the privacy parameters $(\eps, \delta)$. This property is especially important and useful since in practice we rarely want to release only a single statistic about a dataset. Releasing many statistics may require running multiple differentially private algorithms on the same database. Composition is also a very useful tool in algorithm design. In many cases, new differentially private algorithms are created by combining several simpler algorithms. The composition theorems help us analyze the privacy properties of algorithms designed in this way.

Formally, let $\mechanism_0, \mechanism_1, \dots, \mechanism_{k-1}$ be differentially private mechanisms, we define the composition of these mechanisms by independently execute each of them: 
$$
\mechanism(x) 
= \left(\mechanism_0, \dots, \mechanism_{k-1} \right)(x)
= \left(\mechanism_0(x), \dots, \mechanism_{k-1}(x) \right)
$$
where each $\mechanism_i$ is run with independent coin tosses. For example, this is how we might obtain a mechanism answering a $k$-tuple of queries. 

A handful of composition theorems already exist in the literature. The Basic Composition Theorem says that the privacy degrades at most linearly with the number of mechanisms executed. 

\begin{theorem}[Basic Composition \citep{dwork2006our}]
\label{thm:basic-comp}
For every $\eps \ge 0$, $\delta \in [0, 1]$, if $\mechanism_0, \dots, \mechanism_{k-1}$ are each $(\eps, \delta)$-differentially private mechanisms, then the composition $(\mechanism_0, \dots, \mechanism_{k-1})$ is $(k\eps, k\delta)$-differentially private. 
\end{theorem}

Theorem \ref{thm:basic-comp} shows the global privacy degradation is linear in the number of mechanisms in the composition. 
However, if we are willing to tolerate an increase in the $\delta$ term, the privacy parameter $\eps$ only needs to degrade proportionally to $\sqrt{k}$:

\begin{theorem}[Advanced Composition \citep{dwork2010boosting}]
\label{thm:advanced-comp}
For all $\eps \ge 0$, $\delta \in [0, 1]$,
if $\mechanism_0, \dots, \mechanism_{k-1}$ are each $(\eps, \delta)$-differentially private mechanisms and $k < 1/\eps^2$, then for all $\delta' \in (0, 1/2)$, the composition $(\mechanism_0, \dots, \mechanism_{k-1})$ is $ \left(O \left(\sqrt{k \log (1/\delta')} \right) \cdot \eps, k\delta + \delta' \right)$-differentially private. 
\end{theorem}

Theorem \ref{thm:advanced-comp} is an improvement if $\delta' = 2^{-O(k)}$. It can be shown that a degradation function of $\Omega \left(\sqrt{k \log(1/\delta)} \right)$ is necessary even for the simplest differentially private algorithms, such as randomized response \citep{vadhan2017complexity}. 
%\paragraph{Related Work}
%As a building block, differentially private algorithms are often used repeatedly/recursively. 
%Previous works on  composition theorems bound the degradation of privacy when composing DP algorithms sequentially (\textcolor{red}{non-concurrently?}).
%The overall privacy level will degrade as a function of the number of queries and the privacy levels of each DP mechanisms. 
%A simple argument shows that the sequential composition of $k$ queries, each of which is $(\eps_i, \delta_i)$-differentially private, is at least $(\sum_{i=1}^k \eps_i, \sum_{i=1}^k \delta_i)$-differentially private \citep{dwork2006our, dwork2006calibrating, dwork2009differential, dwork2010boosting}, which is commonly referred as \emph{basic composition theorem}.
%A tighter bound under $k$-fold adaptive composition is provided in \citep{dwork2010boosting}, which is commonly referred as \emph{advanced composition theorem}. 
However, despite giving an asymptotically correct upper bound for the global privacy parameter, Theorem \ref{thm:advanced-comp} is not exact. 
\cite{kairouz2015composition} shows how to compute the optimal bound for (non-concurrently) composing $k$ mechanisms where all of them are $(\eps, \delta)$-differentially private.  \cite{murtagh2016complexity} further extends the optimal composition for the more general case of $k$ arbitrary $(\eps_1, \delta_1), \dots, (\eps_k, \delta_k)$-differentially private algorithms, where the privacy parameters may differ for each algorithm in the composition. 
Additionally, making use of the specific properties of the DP algorithms can further improve the privacy composition bound. For example, \emph{moments accountant} is considered in \cite{abadi2016deep}, where they analyzed the privacy of noisy stochastic gradient descent as a composition of subsampled Gaussian mechanism. \cite{dong2020optimal} explored the optimal composition bound over the class of exponential mechanisms. 
%However, all of these techniques implicitly assume that the mechanisms are executed non-concurrently. 
%none of these techniques can directly apply to setting of concurrent composition. 


All of the composition theorems discussed above focus on or implicitly assume that the underlying DP mechanisms are ``one-shot'' algorithms. However, many of the useful differential privacy primitives such as Sparse Vector Technique and Private Multiplicative Weights are actually interactive mechanisms, which allow one to ask an adaptive sequence of queries about the dataset, and a natural question regarding interactive DP mechanisms is whether interactive differential privacy is preserved under a variety of composition operations. Unfortunately, none of results of composition theorems can directly apply to the setting of concurrent compositions, despite that interactive DP algorithms are a more practical choice in the actual deployment of DP mechanisms. To the best of our knowledge, this work is the first to tackle the question of the concurrent compositions of interactive differential privacy. 

We first formalize the notion of an interactive protocol between two parties $A$ and $B$. We do this by viewing each party as a function, taking its private input, all messages it has received, and the party's random coins, to the party's next message to be sent out. 
% Either party can decide to halt the interactive session, and the other party is given an opportunity to compute one more message at that time.

\begin{definition}[Interactive protocols]
An \emph{interactive protocol} $(A, B)$ is any pair of functions. The interaction between $A$ with input $x_A$ and $B$ with input $x_B$ is the following random process (denoted $(A(x_A), B(x_B))$):
\begin{enumerate}
    \item Uniformly choose random coins $r_{A}$ and $r_{B}$ (binary strings) for $A$ and $B$, respectively.
    \item Repeat the following for $i=0, 1, \ldots$: 
    \begin{enumerate}
        \item If $i$ is even, let $m_{i}=A\left(x_A, m_{1}, m_3, \ldots, m_{i-1} ; r_{A} \right)$.
        \item If $i$ is odd, let $m_{i}=B\left(x_B, m_{0}, m_2, \ldots, m_{i-1} ; r_{B} \right)$.
        \item If $m_{i-1} = \halt$, then exit loop.
    \end{enumerate}
\end{enumerate}
\end{definition}
We say $(A, B)$ is an \emph{r-round interactive protocol} if the number of message exchanges is \emph{at most} $2r$. 

We further define the view of a party in an interactive protocol as follows: 
\begin{definition}[View of a party in an interactive protocol]
Let $(A, B)$ be an interactive protocol. $A$'s view of $(A(x_A), B(x_B))$ is the random variable $\View_A \langle A(x_A), B(x_B) \rangle = \left(r_A, x_A, m_{1}, m_3,  \ldots \right)$ consisting of all the messages $m_{1}, m_3, \ldots $ received by $A$ together with the private input $x_A$ and random coins $r_{A}$ for $A$. $B$'s view of $(A(x_A), B(x_B))$ is defined symmetrically. 
\end{definition}

In our case, $A$ is the adversary and $B$ is the mechanism whose input is usually a database $x$. Since $A$ does not have an input in our case, we will denote the interactive protocol as $(A, B(x))$ for the ease of notation.  Since we will only be interested in $A$'s view and $A$ does not have an input, we will drop the subscript and write $A$'s view as $\view{A}{B(x)}$. 

Now we are ready to define the interactive differentially privacy
as a type of interactive protocol between an adversary (without any computational limitations) and an interactive mechanism of special properties. 

\begin{definition}[Interactive Differential Privacy]
A randomized algorithm $\mechanism$ is $(\eps, \delta)$-differentially private interactive mechanism if for every pair of adjacent datasets $x, x'$, for every adversary algorithm $\analyst$, for every possible output set $T \subseteq \range \left( \view{\analyst}{ \mechanism(\cdot) } \right)$ 
we have 
$$
\Pr \left[ \view{\analyst}{\mechanism(x)}  \in T \right] \le e^\eps \Pr \left[ \view{\analyst}{\mechanism(x')} \in T \right] + \delta
$$
where the randomness is over the coin flips of both the algorithm $\mechanism$ and the adversary $\analyst$. 
\end{definition}

Interactive DP mechanism is an important class of DP primitives, as it allows one to ask an adaptive sequence of queries about the dataset. Many of the useful primitives, such as the Sparse Vector Technique \citep{dwork2009complexity, roth2010interactive}, and Private Multiplicative Weights \citep{hardt2010multiplicative} are classic examples of interactive mechanisms. For instance, Sparse Vector Technique are used in adaptive data analysis to prevent overfitting. 
An interactive DP mechanism may allow an adversary make infinite amount of adaptive queries, while making the outputted transcript differentially private. 
Although it seems important, the formal definition of interactive differential privacy was not formulated until recently \citep{gaboardi2020programming}. Having saying that, interactive differentially privacy could be regarded as a special case of \emph{multiparty differential privacy} \citep{beimel2008distributed} if we set the number of parties to 2. 
%A non-interactive mechanism can be viewed as an interactive mechanism that output one response and then terminate the interactive session. 
%The view of the adversary includes both the randomness of the adversary $r$, as well as the responses from the mechanism in each round $(a_1, a_2, \dots,)$. 

Naturally, we can extend the composition procedure described earlier to interactive differentially private mechanisms. The simplest case is when an adversary interact with multiple mechanisms \emph{sequentially}. In this case, all of the composition theorems discussed earlier for non-interactive differential privacy still applies. 
However, a reality strike is that a single adversary could interact with multiple mechanisms \emph{concurrently}, where different threads of interactive sessions can be arbitrarily interleaved with each other. That is, although each response outputs by different mechanisms are generated using individual randomness, the adversary, however, may coordinate the actions it takes in the various executions of interactive sessions, and in particular its actions in one execution may also depend on messages it received in other executions. 

%Table \ref{tb:concurrent-illustration} shows as example of concurrent executions of interactive sessions. 
\begin{comment}
\begin{table}[h!]
\centering
\caption{An example of queries and responses interleaving, where $q_i$ represents query from the adversary to $\mechanism_i$, and $a_i$ represents response from $\mechanism_i$ to the adversary.}
\begin{tabular}{cccc}
$\mechanism_0$ & $\mechanism_1$ &  $\mechanism_2$ \\
$q_0$          &                &                         \\
               & $q_1$          &                         \\
               &                &          $q_2$          \\
               &                &          $a_2$          \\
               & $a_1$          &                         \\
$a_0$          &                &                        
\end{tabular}
\label{tb:concurrent-illustration}
\end{table}
\end{comment}

\paragraph{Concurrent composition in cryptography} 
Although the concurrent composition has not been considered for differential privacy context before, it has been considered for many primitives in cryptography, and it is often much more subtle than the sequential composition \citep{Dolev91, richardson1999concurrent, dwork2004concurrent, pass2008concurrent}. 
For example, standard zero-knowledge protocols are no longer zero-knowledge when a single prover is involved in multiple, simultaneous zero-knowledge proofs with one or multiple verifiers \citep{richardson1999concurrent}. 

\section{Main Results}
In this paper, we use $\concomp(\mechanism_0, \dots, \mechanism_{k-1})$ to denote the concurrently composed mechanism of $\mechanism_0, \dots, \mechanism_{k-1}$, in order to distinguish with the sequentially composed mechanism or the composition of non-interactive mechanisms.
We begin by extending the results of basic composition theorem to the interactive case. 

\begin{restatable}[Basic Composition of Pure Interactive Differential Privacy]{theorem}{concompbasicpure}
\label{thm:concomp-basic}
If interactive mechanisms $\mechanism_0, \dots, \mechanism_{k-1}$ are each $(\eps_i, 0)$-differentially private, then their concurrent composition $\concomp(\mechanism_0, \ldots, \mechanism_{k-1})$ is $\left(\sum_{i=0}^{k-1} \eps_i, 0 \right)$-interactive differentially private. 
\end{restatable}

Theorem \ref{thm:concomp-basic} only applies to the case when $\delta=0$. Our next result gives a privacy bound for the case of $\delta > 0$. 

%\begin{restatable}{theorem}{concompbasicapprox}
%\label{thm:bound-pointwise}
%If $\mechanism_0, \dots, \mechanism_{k-1}$ are each $(\eps_i, \delta_i)$ differentially private, then the concurrent composition of $\concomp(\mechanism_0, \dots, \mechanism_{k-1})$ is $(\sum_{i=0}^{k-1} \eps_i,  \frac{2}{1-e^{-\sum_{i=0}^{k-1} \eps_i}} \sum_{i=0}^{k-1} \delta_i )$-differentially private. 
%\end{restatable}

\begin{restatable}{theorem}{concompbasicapprox}
\label{thm:concomp-basic-approx}
Let $\sigma: \{0, 1, \ldots, n-1\} \rightarrow \{0, 1, \ldots, n-1\}$ be any permutation of $0, \ldots, n-1$. 
If interactive mechanisms $\mechanism_0, \dots, \mechanism_{k-1}$ are each $(\eps_i, \delta_i)$-differentially private, then their concurrent composition $\concomp(\mechanism_0, \ldots, \mechanism_{k-1})$ is
$\left(\sum_{i=0}^{k-1} \eps_i, \delta_g \right)$-differentially private, where 
$$
\delta_g = \min_{\sigma} 
\left( 
\delta_{\sigma(0)} + \sum_{i=1}^{k-1} e^{\sum_{j=0}^{i-1}\eps_{\sigma(j)}} \delta_{\sigma(i)} 
\right)
$$
For mathematical convenience, we use an upper bound for $\delta_g$ in practice and $\concomp(\mechanism_0, \ldots, \mechanism_{k-1})$ is $\left( \sum_{i=0}^{k-1} \eps_i, k e^{\sum_{i=0}^{k-1} \eps_i} \max_i(\delta_i) \right)$-differentially private.
\end{restatable}

The above theorem may also suggest that the basic composition theorem might be worse in $\delta$ for the interactive case, in comparison with the linearly increasing $\delta$ in Theorem \ref{thm:basic-comp}. 

\cite{kairouz2015composition} shows that every (non-interactive) $(\eps, \delta)$-DP mechanism can be simulated by randomized response, which is the basis for analysing the exact composition bound for non-interactive differential privacy. We show a similar result for the pure interactive DP mechanisms, which reduces the interactive mechanisms to non-interactive mechanisms, and we derive the \emph{optimal} bound for the concurrent composition theorem for pure DP mechanisms accordingly. 

\begin{restatable}{theorem}{reducenonint}
\label{thm:bound-opt}
If $\mechanism_0, \dots, \mechanism_{k-1}$ are each $(\eps_i, 0)$-differentially private, then given the target security parameter $\delta_g$, the privacy parameter of concurrent composition $\concomp(\mechanism_0, \dots, \mechanism_{k-1})$ is
upper bounded by the least value of $\varepsilon_{g} \geq 0$ such that
$$
\frac{1}{\prod_{i=0}^{k-1}\left(1+\mathrm{e}^{\varepsilon_{i}}\right)} 
\sum_{S \subseteq\{0, \ldots, k-1\}} \max 
\left
\{\mathrm{e}^{\sum_{i \in S} \varepsilon_{i}}-\mathrm{e}^{\varepsilon_{g}} \cdot \mathrm{e}^{\sum_{i \notin S} \varepsilon_{i}}, 0
\right\} 
\leq \delta_g
$$
A special case when all $\mechanism_0, \dots, \mechanism_{k-1}$ are $(\eps, \delta)$-differentially private, then privacy parameter is upper bounded by the least value of $\eps_g \ge 0$ such that
$$
\frac{1}{\left(1+\mathrm{e}^{\varepsilon}\right)^k} 
\sum_{i=0}^k {k \choose i} 
\max 
\left
\{\mathrm{e}^{i \eps }-\mathrm{e}^{\varepsilon_{g}} \cdot \mathrm{e}^{(k-i) \varepsilon}, 0
\right\} 
\leq \delta_g
$$
\end{restatable}



==> pureDP.tex <==
In this section, we show that for pure differential privacy, the privacy bound for concurrent composition is the same as for sequential or non-interactive composition. 
The proof idea is that in an interactive protocol where the adversary is concurrently interacting with multiple mechanisms, its interaction with one particular mechanism could be viewed as the combination of the adversary and the remaining mechanisms interacting with that mechanism, and the differential privacy guarantee still holds for the ``combined adversary''.

\newcommand{\indis}[2]{\stackrel{( #1 , #2 )}{\approx}}

A useful notation for thinking about differential privacy and simplify presentations is defined below. 
\begin{definition}
Two random variables $Y$ and $Z$ taking values in the same output space $\mathcal{Y}$ is \emph{$(\eps, \delta)$-indistinguishable} if for every event $T \subseteq \mathcal{Y}$, we have:
$$
\Pr[Y \in T] \le e^\eps \Pr[Z \in T] + \delta
$$
$$
\Pr[Z \in T] \le e^\eps \Pr[Y \in T] + \delta
$$
which is denoted as $Y \indis{\eps}{\delta} Z$. 
\end{definition}
Notice that an algorithm $\mechanism$ is $(\eps, \delta)$ differentially private if and only if for all pairs of adjacent datasets $x, x'$, we have $\mechanism(x) \indis{\eps}{\delta} \mechanism(x')$. 

\begin{lemma}[\cite{vadhan2017complexity}]
For random variables $X, Y, Z$, if $X \indis{\eps_1}{0} Y$, $Y \indis{\eps_2}{0} Z$, then $X \indis{\eps_1+\eps_2}{0} Z$. 
\end{lemma}

\concompbasicpure*

\begin{proof}
We first consider the simplest case that $\analyst$ concurrently interact with 2 mechanisms $\mechanism, \Tilde{\mechanism}$, and then extend the result to general amount of mechanisms. 
Suppose $\mechanism$ and $\Tilde{\mechanism}$ are each $(\eps, 0)$ and $(\Tilde{\eps}, 0)$-differentially private interactive mechanisms. 
Denote the messages received by $\analyst$ from $\mechanism$ as $(a_0, a_1, \dots, )$, and the messages received by $\analyst$ from $\Tilde{\mechanism}$ as $(\Tilde{a}_0, \Tilde{a}_1, \dots,)$. Due to Lemma \ref{lemma:ordered}, we can WLOG assume $\analyst$ alternates messages between $\mechanism$ and $\Tilde{\mechanism}$, i.e., the sequence of messages $\analyst$ received is $(a_0, \Tilde{a}_0, a_1, \Tilde{a}_1, \dots, )$. 
We use $r_\analyst$, $r_{\mechanism}, r_{\Tilde{\mechanism}}$ to denote the random coin tosses for $\analyst$, $\mechanism$, and $\Tilde{\mechanism}$, respectively. We can view $\analyst$ and $\Tilde{\mechanism}(x)$ as a single adversary $\analyst^*_{\Tilde{\mechanism}}(x)$ interacting with $\mechanism(x)$ defined as follows: 
\begin{enumerate}
    \item Random coin tosses for $\analyst^*_{\Tilde{\mechanism}}(x)$ consist of $r = (r_\analyst, r_{\Tilde{\mechanism}})$. 
    \item $\analyst^*_{\Tilde{\mechanism}}(x)(a_0, a_1, \dots, a_{i-1}; r)$ is computed as follows: 
    \begin{enumerate}
        \item $\Tilde{q}_{i-1} = \analyst(a_0, \Tilde{a}_0, 
        a_1, \Tilde{a}_1, \dots, a_{i-1}; r_\analyst)$. %, send to $\Tilde{\mechanism}$. 
        \item $\Tilde{a}_{i-1} = \Tilde{\mechanism}(x, \Tilde{q}_0, \Tilde{q}_1, \dots, \Tilde{q}_{i-1}; r_{\Tilde{\mechanism}})$. %, send to $\analyst$.
        \item $q_i = \analyst(a_0, \Tilde{a}_0, \dots, a_{i-1}, \Tilde{a}_{i-1}; r_\analyst)$. 
        \item Output $q_i$.  
    \end{enumerate}
\end{enumerate}


%For every $\analyst$ and every fixed message sequence $(\Tilde{a}_1, \Tilde{a}_2, \dots, )$ we can construct a new strategy $\analyst^*_{\Tilde{\mechanism}}$ whose randomness depends on both $\analyst$'s randomness and $\Tilde{a}_1, \Tilde{a}_2, \dots$ (the randomness of $\Tilde{\mechanism}$ is reflected in the variable of transcript). 
%We can view $\analyst^*_{\Tilde{\mechanism}}$ as knowing the entire message sequence $\Tilde{a}_1, \Tilde{a}_2, \dots$ in advance, but only making its $i$th query strategy to $\mechanism_1$ based on the randomness of $\analyst$ and messages $\Tilde{a}_1, \dots,  \Tilde{a}_{i-1}$. 

We can see that $\analyst^*_{\Tilde{\mechanism}}(x)$ is a well-defined strategy throughout the entire interactive protocol with $\mechanism$, where the randomness of $\analyst^*_{\Tilde{\mechanism}}(x)$ is fixed as $(r_\analyst, r_{\Tilde{\mechanism}})$. 
Given a transcript of $\analyst^*_{\Tilde{\mechanism}}(x)$'s view $(r_{\analyst}, r_{\Tilde{\mechanism}}, x, a_0, a_1, \dots, )$, we can recover the corresponding transcript of $\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))}$ through the following post-processing algorithm $\postprocessing$, which is defined as follows: 

$\postprocessing \left(r_{\analyst}, r_{\Tilde{\mechanism}}, a_0, a_1, \dots, a_{T-1} \right)$:
\begin{enumerate}
    \item For $i = 1 \dots T-1$, compute  
    \begin{enumerate}
        \item $\Tilde{q}_{i-1} = \analyst(a_0, \Tilde{a}_0, \dots, a_{i-1}; r_{\analyst})$
        \item $\Tilde{a}_{i-1} = \Tilde{\mechanism}(x, \Tilde{q}_1, \Tilde{q}_2, \dots, \Tilde{q}_{i-1}; r_{\Tilde{\mechanism}})$
    \end{enumerate}
    \item Output $(r_{\analyst}, a_0, \Tilde{a}_0, \dots, a_{T-1}, \Tilde{a}_{T-1})$. 
\end{enumerate}

\noindent Observe that for every $\left(x, r_\analyst, r_\mechanism, r_{\Tilde{\mechanism}}\right)$, 
\begin{align}
&\postprocessing \left( \view{\analyst^*_{\Tilde{\mechanism}}(x; r_\analyst, r_{\Tilde{\mechanism}})}{\mechanism(x; r_\mechanism)} \right) \nonumber \\
&= \view{\analyst(r_\analyst)}{\concomp(\mechanism(x; r_\mechanism), \Tilde{\mechanism}(x; r_{\Tilde{\mechanism}}))} \nonumber
\end{align}
%For notation clarity, we will simply write $\postprocessing(r_{\analyst}, r_{\Tilde{\mechanism}}, a_0, a_1, \dots, a_{T-1})$ when the adversary and mechanisms are clear from the context. 
%By slightly abusing the notation, for a subset $T \subseteq \range(\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))})$ we denote $\postprocessing^{-1}(T) = \{ z \in \view{\analyst^*_{\Tilde{\mechanism}}(x)}{\mechanism(x)} | \postprocessing(z) \in T \}$. 
Therefore we have 
%\begin{align}
%&\Pr \left[
%\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \in T \right] \nonumber \\
%&= \Pr \left[
%\view{\analyst^*_{\Tilde{\mechanism}}(x)}{\mechanism(x)} \in \postprocessing^{-1}(T) \right] \nonumber
%\end{align}
\begin{align}
    &\Pr \left[ \view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \in T \right] \nonumber \\
    &\equiv \postprocessing \left(
\view{ \analyst^*_{\Tilde{\mechanism}}(x) }{\mechanism(x)}
\right) \nonumber
\end{align}

for every $T \subseteq \range(\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))})$. 

Since $\mechanism$ is $\eps$-differentially private, we know that 
$$
\view{ \analyst^*_{\Tilde{\mechanism}}(x) }{\mechanism(x)}
\indis{\eps}{0}
\view{ \analyst^*_{\Tilde{\mechanism}}(x) }{\mechanism(x')}
$$
which leads to 
\begin{align}
&\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \nonumber \\
&\equiv 
\postprocessing \left(
\view{ \analyst^*_{\Tilde{\mechanism}}(x) }{\mechanism(x)}
\right) \nonumber \\
&\indis{\eps}{0}
\postprocessing \left(
\view{ \analyst^*_{\Tilde{\mechanism}}(x) }{\mechanism(x')}
\right) \nonumber \\
&\equiv \view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \nonumber
\end{align}

\begin{comment}
    for every possible subset $T \subseteq \range(\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))})$, 
    \begin{align}
    &\log \left( \frac{
    \Pr \left[
    \view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \in T \right] }{\Pr \left[ \view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \in T \right]} \right) \nonumber \\
    &=
    \log \left( \frac{ 
    \Pr \left[
    \view{\analyst^*_{\Tilde{\mechanism}}(x)}{\mechanism(x)} = \postprocessing^{-1}(T) \right]}{
    \Pr \left[
    \view{\analyst^*_{\Tilde{\mechanism}}(x)}{\mechanism(x')} = \postprocessing^{-1}(T) \right]} \right) \nonumber \\
    &\le \eps \nonumber
    \end{align}
    since $\mechanism$ is $\eps$-differentially private. 
\end{comment}

Symmetrically, we can obtain
\begin{align}
&\view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \nonumber \\
&\indis{\Tilde{\eps}}{0} 
\view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x'))} \nonumber
\end{align}

\begin{comment}
    \begin{align}
    &\log \left( \frac{
    \Pr \left[
    \view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \in T \right]}{ 
    \Pr \left[
    \view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x'))} \in T
    \right]
    } \right) \nonumber \\
    &=
    \log \left( \frac{ 
    \Pr \left[
    \view{\analyst^*_{\mechanism}(x')}{\Tilde{\mechanism}(x)} = \postprocessing^{-1}(T) \right]}{
    \Pr \left[
    \view{\analyst^*_{\mechanism}(x')}{\Tilde{\mechanism}(x')} = \postprocessing^{-1}(T) \right]} \right) \nonumber \\
    &\le \Tilde{\eps} \nonumber
    \end{align}
\end{comment}

Therefore, %for every subset $T \subseteq \range(\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))})$,
we have 
\begin{align}
&\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \nonumber \\
&\indis{\eps + \Tilde{\eps}}{0} 
\view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x'))} \nonumber
\end{align}

\begin{comment}
    \begin{align}
    & \log \left( \frac{\view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \in T}{\view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x'))} \in T} \right) \nonumber \\
    &= 
    \log \left(
    \frac{
    \Pr[
    \view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \in T]}{
    \Pr[
    \view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \in T]} \right. \nonumber \\
    & \left.
    ~~~~~~~~~~~\cdot \frac{
    \Pr[
    \view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \in T]}{
    \Pr[
    \view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \in T]}
    \right) \nonumber \\
    &= \log \left(
    \frac{
    \Pr[
    \view{\analyst}{\concomp(\mechanism(x), \Tilde{\mechanism}(x))} \in T]}{
    \Pr[
    \view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \in T]} \right) \nonumber \\
    &+ \log \left( \frac{
    \Pr[
    \view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x))} \in T]}{
    \Pr[
    \view{\analyst}{\concomp(\mechanism(x'), \Tilde{\mechanism}(x'))} \in T]} \right) \nonumber \\
    &\le \eps + \Tilde{\eps} \nonumber
    \end{align}
\end{comment}

The result can be easily extended to the case when more than 2 mechanisms are concurrently composed by induction.  Therefore 
for every $\eps_i \ge 0$, if interactive mechanism $\mechanism_i$ is $(\eps_i, 0)$-differentially private for $i=0, \dots, k-1$, then the concurrent composition $\concomp(\mechanism_0, \dots, \mechanism_{k-1})$ is $\left(\sum_{i=0}^{k-1} \eps_i, 0\right)$-differentially private. 
\end{proof}

This result tells us that even under concurrent composition, the privacy parameters of the resulting composed mechanisms are the ``sum up'' of the individual algorithms for the case pure differential privacy. 




==> technicalPre.tex <==



The formal definition of the concurrent composition of interactive protocols is provided here. 

\begin{definition}[Concurrent Composition of Interactive Protocols]
Let $\mechanism_0, \dots, \mechanism_{k-1}$ be interactive mechanisms. We say $\mechanism = \concomp(\mechanism_0, \dots, \mechanism_{k-1})$ is the \emph{concurrent composition} of mechanisms $\mechanism_0, \dots, \mechanism_{k-1}$ if $\mechanism$ runs as follows:
\begin{enumerate}
    \item Random coin tosses for $\mechanism$ consist of $r=(r_0, \dots, r_{k-1})$ where $r_j$ are random coin tosses for $\mechanism_j$. 
    \item Inputs for $\mechanism$ consists of $x=(x_0, \dots, x_{k-1})$ where $x_j$ is private input for $\mechanism_j$. 
    \item $\mechanism(x, m_0, \dots, m_{i-1}; r)$ is defined as follows: 
    \begin{enumerate}
        \item Parse $m_{i-1}$ as $(q, j)$ where $q$ is a query and $j \in [k]$. If $m_{i-1}$ cannot be parsed correctly, output \halt. 
        \item Extract history $(m_0^j, \dots, m_{t-1}^j)$ from $(m_0, \dots, m_{i-1})$ where $m_i^j$ are all of the queries to mechanism $\mechanism_j$. 
        \item Output $\mechanism_j(x_j, m_0^j, \dots, m_{t-1}^j; r_j)$. 
    \end{enumerate}
\end{enumerate}
\end{definition}

For the convenience of the proof, we introduce a variant of concurrent composition of interactive protocols, which only accept queries in the exact order of $\mechanism_0, \dots, \mechanism_{k-1}$. 

\begin{definition}[Ordered Concurrent Composition of Interactive Protocols]
Let $\mechanism_0, \dots, \mechanism_{k-1}$ be interactive mechanisms. 
We say $\mechanism = \concomp_{\order}(\mechanism_0, \dots, \mechanism_{k-1})$ is the \emph{ordered concurrent composition} of mechanisms $\mechanism_0, \dots, \mechanism_{k-1}$ if $\mechanism(x)$ runs as follows:
\begin{enumerate}
    \item Random coin tosses and inputs for $\mechanism$ are the same as $\concomp(\mechanism_0, \dots, \mechanism_{k-1})$. 
    \item $\mechanism(x, m_0, \dots, m_{i-1}; r)$ is defined as follows: 
    \begin{enumerate}
        \item Let $j = i \bmod k$, $t = \lfloor i/k\rfloor$.
        \item Output $\mechanism_j(x, m_j,m_{j+k}, \ldots, m_{j+t\cdot k};r_j)$.
    \end{enumerate}
\end{enumerate}
\end{definition}

We also introduce a special kind of interactive mechanism, which ignores all query strings begin with 0. 
\begin{definition}[Null-query Extension]
Given an interactive mechanism $\mechanism$, define its {\em null-query extension} $\mechanism^\emptyset$ defined as follows: For any input message sequence $m$, 
$\mechanism^\emptyset(x,m;r)=\mechanism(x,m';r)$ where $m'=(m'_1,\ldots,m'_k)$ such that $(1m'_1,\ldots,1m'_k)$ is the subsequence of
$m$ consisting of all strings that begin with bit 1. That is, all messages that begin with 0 are ``null queries'' that are ignored. 
By convention, $\mechanism(x,\lambda;r)=\bot$ where $\lambda$ is an empty tuple. 
\end{definition}

Now we show that in order to prove $\concomp(\mechanism_0, \dots, \mechanism_{k-1})$ is $(\eps, \delta)$-differentially private, it suffices to prove a corresponding ordered concurrent composition is also $(\eps, \delta)$-differentially private. 
We use $X \equiv Y$ to denote that two random variables $X$ and $Y$ have the same distribution. 

\begin{lemma}
$\concomp(\mechanism_0, \dots, \mechanism_{k-1})$ is an $(\eps, \delta)$-differentially private interactive mechanism if the ordered concurrent composition of the null-query extensions of $\mechanism_0, \dots, \mechanism_{k-1}$, i.e.,\\ $\concomp_{\order}(\mechanism^\emptyset_1, \dots, \mechanism^\emptyset_k)$, is an $(\eps, \delta)$-differentially private interactive mechanism.
\label{lemma:ordered}
\end{lemma}
\begin{proof}
Suppose $\concomp_{\order}\left(\mechanism^\emptyset_0, \dots, \mechanism^\emptyset_{k-1}\right)$ is $(\eps, \delta)$-differentially private. 
For every adversary $\analyst$ interacting with $\concomp \left(\mechanism_0, \dots, \mechanism_{k-1} \right)$, 
we construct another adversary $\analyst'$ interacting with $\concomp_\order(\mechanism_0^\emptyset, \dots, \mechanism_{k-1}^\emptyset)$ as follows: 
given any settings of coin tosses $r$, and any history $(q_0, a_0, \dots, q_{i-1}, a_{i-1})$ between $\analyst$ and $\concomp(\mechanism_0, \dots, \mechanism_{k-1})$,
\begin{enumerate}
    \item Let $q_i = \analyst(a_0, \dots, a_{i-1}; r)$.
    \item Parse $q_{i-1}$ as $(q_{i-1}^*, s)$ where $q_{i-1}^*$ is a query and $s \in \{0, \dots, k-1\}$ the index of target mechanism. Parse $q_{i}$ as $(q_{i}^*, t)$ in a similar way. 
    \item %Let $\nullquery$ be any strings that are distinct from all messages that $\mechanism_0, \dots, \mechanism_{k-1}$ accepts. 
    Send the null query $0$ to $\mechanism_{(s+1)\mod k}^\emptyset, \dots, \mechanism_{(t-1)\mod k}^\emptyset$ in order. %If $s \ge t$, send $0$ to $\mechanism_0^\emptyset$ after sending to $\mechanism_{k-1}^\emptyset$. 
    \item Send $1q_i^*$ to $\mechanism_t^\emptyset$. 
\end{enumerate}
Write $\mechanism = \concomp(\mechanism_0, \dots, \mechanism_{k-1})$, and $\mechanism' = \concomp_{\order}(\mechanism_0^\emptyset, \dots, \mechanism_{k-1}^\emptyset)$. 
For every query sequence $q$ from $\analyst$, we have $\mechanism(x, q; r) = \mechanism'(x, q'; r)$ where $q'$ is the sequence of queries that $\analyst'$ asks based on $q$ (with `1' in front of every query in $q$ and additional $0$s). 
Therefore, for every $\analyst$ interact with $\mechanism$, and for every dataset $x$ we have 
$$
\view{\analyst}{\mechanism(x)} \equiv \postprocessing(
\view{\analyst'}{\mechanism'(x)})
$$
where $\postprocessing$ refers to remove all repeated answers from the null query. 
This immediately leads to 
\begin{align}
&\Pr[ \view{\analyst}{\mechanism(x)} \in T] \nonumber \\
&= 
\Pr[ \postprocessing( \view{\analyst'}{\mechanism'(x)}) \in T] \nonumber \\
&\le e^\eps \Pr[ \postprocessing(\view{\analyst'}{\mechanism'(x')}) \in T] + \delta \nonumber \\
&= e^\eps \Pr[ \view{\analyst}{\mechanism(x')} \in T] + \delta \nonumber
\end{align}

Therefore, $\mechanism$ is also $(\eps, \delta)$-DP. 
\end{proof}

Given Lemma \ref{lemma:ordered}, for all of the concurrent compositions we considered in this paper, we assume that the concurrent compositions are ordered. For example, if an adversary $\analyst$ is concurrently interacting with two mechanisms $\concomp(\mechanism_0, \mechanism_1)$, we assumes that the queries are alternates between $\mechanism_0$ and $\mechanism_1$. 


